A categorification of the stable SU(2) Witten-Reshetikhin-Turaev invariant of links in S2 x S1

The WRT invariant of a link L in S2xS1 at sufficiently high values of the level r can be expresses as an evaluation of a special polynomial invariant of L at 2r-th root of unity. We categorify this polynomial invariant by associating to L a bigraded homology whose graded Euler characteristic is equal to this polynomial. If L is presented as a closure of a tangle in S2xS1, then the homology of L is defined as the Hochschild homology of the H_n-bimodule associated to the tangle by M. Khovanov. This homology can also be expressed as a stable limit of Khovanov homology of the circular closure of the tangle in S3 through the torus braid with high twist.

==> defs/locdef.tex <==
\def\xI{I}
\def\xJ{J}
\def\xK{K}
\def\xL{L}
\def\xM{M}
\def\xN{N}

\def\xrI{ \bar{\xI} }
\def\xrJ{ \bar{\xJ} }
\def\xrK{ \bar{\xK} }
\def\xrL{ \bar{\xL} }
\def\xrM{ \bar{\xM} }
\def\xrN{ \bar{\xN} }

%\def\xi{ i }
\def\xj{ j }
\def\xk{ k }
\def\xl{ l }
\def\xm{ m }
\def\xn{ n }

\def\xri{ \bar{\xi} }
\def\xrj{ \bar{\xj} }
\def\xrk{ \bar{\xk} }
\def\xrl{ \bar{\xl} }
\def\xrm{ \bar{\xm} }
\def\xrn{ \bar{\xn} }

\def\xip{ \xi\p }
\def\xjp{ \xj\p }
\def\xkp{ \xk\p }
\def\xlp{ \xl\p }
\def\xmp{ \xm\p }
\def\xnp{ \xn\p }

\def\xrip{ \xri\p }
\def\xrjp{ \xrj\p }
\def\xrkp{ \xrk\p }
\def\xrlp{ \xrl\p }
\def\xrmp{ \xrm\p }
\def\xrnp{ \xrn\p }

\def\xA{ A }
\def\xB{ B }
\def\xC{ C }
\def\xD{ D }
\def\xE{ E }
\def\xF{ F }

\def\xrA{ \bar{\xA} }
\def\xrB{ \bar{\xB} }
\def\xrC{ \bar{\xC} }
\def\xrD{ \bar{\xD} }
\def\xrE{ \bar{\xE} }
\def\xrF{ \bar{\xF} }

\def\xa{ a }
\def\xb{ b }
\def\xc{ c }
\def\xd{ d }
\def\xe{ e }
\def\xf{ f }

\def\xra{ \bar{\xa} }
\def\xrb{ \bar{\xb} }
\def\xrc{ \bar{\xc} }
\def\xrd{ \bar{\xd} }
\def\xre{ \bar{\xe} }
\def\xrf{ \bar{\xf} }

\def\xmu{ \mu }
\def\xnu{ \nu }
\def\xrho{ \rho }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\BRST{BRST}
\def\Ec{Inter-fiber connection}
\def\aEc{a \Ec}
\def\thEc{the \Ec}

\def\Bth{B-theory}

\def\Fc{fibration connection}

\def\hK{hyper-K\"{a}hler}
\def\pbk{pull-back}

\def\LC{Levi-Civita}
\def\LCc{\LC\ connection}

\def\cvdr{covariant derivative}
\def\cvdrs{\cvdr s}


\def\yX{ X }
\def\yY{ Y }
\def\yZ{ Z }
\def\yW{ W }

\def\yN{ n }
\def\yM{ m }

\def\yeta{ \eta }
\def\ychi{ \chi }

\def\yetav#1{ \yeta^{\bar{#1}} }
\def\yetaI{ \yetav{\xI} }
\def\yetaJ{ \yetav{\xJ} }
\def\yetai{ \yetav{\xi} }
\def\yetaj{ \yetav{\xj} }

\def\ychiv#1#2{ \ychi_{#1}^{#2} }
\def\ychim#1{ \ychiv{\xmu}{#1} }
\def\ychin#1{ \ychiv{\xnu}{#1} }
\def\ychir#1{ \ychiv{\xrho}{#1} }

\def\ychimI{ \ychim{\xI} }
\def\ychimi{ \ychim{\xi} }

\def\lrbcb#1{ \big( #1 \big) }

\def\LVbr#1#2#3{ [\zV_{#1},#2]^{#3} }
\def\LVdr{ \mathrm{L}_{\zV} }
\def\LVdrv#1{ \lrbcb{ \LVdr #1} }


\def\xee{\begin{equation}}
\def\yee{\end{equation}}


\def\mtg{ \mathrm{g} }
\def\mtgv#1#2{ \mtg_{#1\bar{#2}} }
\def\mtgij{ \mtgv{\xi}{\xj} }
\def\mtgIJ{ \mtgv{\xI}{\xJ} }
\def\mtgab{ \mtgv{\xa}{\xb} }

\def\mtgiv#1#2{ \mtg^{\bar{#1}#2} }

\def\xCG{ \Gamma }
\def\CGv#1#2#3{ \xCG^{#1}_{#2#3} }
\def\CGijk{ \CGv{\xi}{\xj}{\xk} }

\def\xCg{ \gamma }
\def\Cgv#1#2#3{ \xCg^{#1}_{#2#3} }
\def\Cgabc{ \Cgv{\xa}{\xb}{\xc} }

\def\yCg{ \gamma }
\def\yCgv#1#2#3{ \yCg^{#1}_{#2#3} }
\def\yCgijk{ \yCgv{\xi}{\xj}{\xk} }

\def\RR{ \mathrm{R} }
\def\RRv#1#2#3#4{ \RR^{#1}_{#2#3\bar{#4}}}
\def\RRJKLM{ \RRv{\xJ}{\xK}{\xL}{\xM} }
\def\RRabcd{ \RRv{\xa}{\xb}{\xc}{\xd} }

\def\cRR{ \mathcal{R} }
\def\cRRv#1#2#3#4{ \cRR^{#1}_{#2#3\bar{#4}}}
\def\cRRABCD{ \cRRv{\xA}{\xB}{\xC}{\xD} }

\def\ER{ \mathrm{R} }
\def\ERv#1#2#3{ \ER^{#1}_{#2\bar{#3}} }
\def\ERaij{ \ERv{\xa}{\xi}{\xj} }

\def\ERsv#1#2#3{ \ER^{#1}_{#2#3} }
\def\ERbv#1#2#3{ \ER^{\bar{#1}}_{\bar{#2}#3} }
\def\ERsbv#1#2#3{ \ER^{\bar{#1}}_{\bar{#2}\bar{#3}} }

\def\ERsaij{ \ERsv{\xa}{\xi}{\xj} }

\def\ERbaij{ \ERbv{\xa}{\xi}{\xj} }

\def\delv#1{ \del_{#1}\, }
\def\delm{ \delv{\xmu} }
\def\deln{ \delv{\xnu} }
\def\delr{ \delv{\xrho} }
\def\delth{ \delv{3} }

\def\nblv#1{ \nabla_{#1} }
\def\nblmu{ \nblv{\xmu} }

\def\tnbl{ \tilde{\nabla} }
\def\tnblv#1{ \tnbl_{#1} }

\def\xpar{ \parallel }
\def\xprp{ \perp }

\def\nblpar{ \nabla^\xpar }
\def\nblprp{ \nabla^\xprp }
\def\nblparv#1{ \nblpar_{#1} }
\def\nblprpv#1{ \nblprp_{#1} }
\def\nblpara{ \nblparv{\xa} }
\def\nblprpi{ \nblprpv{\xi} }

\def\mrQ{ \mathrm{Q} }
\def\dltQ{ \delta_{\mrQ} }
\def\dltQb#1{ \dltQ\lrbcb{#1} }

\def\xve{ v }
\def\xom{ \omega }
\def\vfv#1{ \xve^{#1} }
\def\vfa{ \vfv{\xa} }
\def\omfv#1{ \xom_{#1} }

\def\vfa{ \vfv{\xa} }
\def\vfb{ \vfv{\xb} }
\def\vfc{ \vfv{\xc} }
\def\vfi{ \vfv{\xi} }

\def\vpar{ \xve_{\xpar} }
\def\vprp{ \xve_{\xprp} }

\def\vparv#1{ \vpar^{#1} }
\def\vprpv#1{ \vprp^{#1} }

\def\vpara{ \vparv{\xa} }
\def\vparb{ \vparv{\xb} }
\def\vparc{ \vparv{\xc} }
\def\vprpi{ \vprpv{\xi} }

\def\xwe{ w }
\def\wfv#1{ \xwe^{#1} }
\def\wfA{ \wfv{\xA} }

\def\wpar{ \xwe_{\xpar} }
\def\wprp{ \xwe_{\xprp} }
\def\wparv#1{ \wpar^{#1} }
\def\wprpv#1{ \wprp^{#1} }

\def\wpara{ \wparv{\xa} }
\def\wprpi{ \wprpv{\xi} }

\def\xphi{ \phi }
\def\xphiv#1{ \phi^{#1} }
\def\xphiI{ \xphiv{\xI} }
\def\xphirJ{ \xphiv{\xrJ} }
\def\xphia{ \xphiv{\xa} }
\def\xphirb{ \xphiv{\xrb} }
\def\xphij{ \xphiv{\xj} }
\def\xphirj{ \xphiv{\xrj} }

\def\yN{ n }
\def\yM{ m }

\def\zV{ V }
\def\zVv#1#2{ \zV^{#1}_{#2} }
\def\zVai{ \zVv{\xa}{\xi} }

\def\zVrv#1#2{ \zVv{\bar{#1}}{\bar{#2}} }
\def\zVrai{ \zVrv{\xa}{\xi} }

\def\zVbv#1#2{ \zV^{\bar{#1}}_{\bar{#2}} }


\def\bulk{ \mathrm{bulk} }
\def\bndr{ \mathrm{bndr} }
\def\Lgr{ \mathcal{L} }
\def\Lgrv#1{ \Lgr_{#1} }
\def\Lgro{ \Lgrv{1} }
\def\Lgrt{ \Lgrv{2} }

\def\Lgrb{ \Lgr^\bulk }
\def\Lgrbv#1{ \Lgrb_{#1} }
\def\Lgrbo{ \Lgrbv{1} }
\def\Lgrbt{ \Lgrbv{2} }

\def\Lgrn{ \Lgr^\bndr }
\def\Lgrnv#1{ \Lgrn_{#1} }
\def\Lgrno{ \Lgrnv{1} }
\def\Lgrnt{ \Lgrnv{2} }


\def\Vgr{ \mathcal{V} }
\def\Vgrv#1{ \Vgr_{#1} }
\def\Vgro{ \Vgrv{1} }
\def\Vgrt{ \Vgrv{2} }

\def\Vgrb{ \Vgr^\bulk }
\def\Vgrbv#1{ \Vgrb_{#1} }
\def\Vgrbo{ \Vgrbv{1} }
\def\Vgrbt{ \Vgrbv{2} }

\def\Vgrn{ \Vgr^\bndr }
\def\Vgrnv#1{ \Vgrn_{#1} }
\def\Vgrno{ \Vgrnv{1} }
\def\Vgrnt{ \Vgrnv{2} }

\def\Tng{ \mathrm{T} }
\def\Tngv#1{ \Tng^{#1} }
\def\Tngpar{ \Tngv{\xpar} }
\def\Tngprp{ \Tngv{\xprp} }


\def\cA{ \mathcal{A} }
\def\cAv#1#2#3{ \cA^{#1}_{#2#3} }
\def\cAABC{ \cAv{\xA}{\xB}{\xC} }
\def\tcA{ \tilde{\cA} }
\def\tcAv#1#2#3{ \tcA^{#1}_{#2#3} }
\def\tcAABC{ \tcAv{\xA}{\xB}{\xC} }

\def\trT{ \mathcal{T} }
\def\trTv#1#2#3{ \trT^{#1}_{#2#3} }
\def\trTABC{ \trTv{\xA}{\xB}{\xC} }
\def\trTajk{ \trTv{\xa}{\xj}{\xk} }

\def\yveps{ \varepsilon }
\def\yvepsmnr{ \yveps_{\xmu\xnu\xrho} }
\def\yvepsmn{ \yveps_{\xmu\xnu} }
\def\yeps{ \epsilon }
\def\yepsv#1#2{ \yeps_{#1#2} }
\def\yepsIJ{ \yepsv{\xI}{\xJ} }
\def\yepsKJ{ \yepsv{\xK}{\xJ} }

\def\yepsiv#1#2{ \yeps^{#1#2} }

\def\mpi{ \pi }
\def\mpiv#1{ \mpi_{#1} }
\def\mpiphiI{ \mpiv{\xphiI} }
\def\mpiphirJ{ \mpiv{ \xphirJ} }


\def\wEta{ H }
\def\wEtav#1{ \wEta^{\bar{#1}} }
\def\wEtaA{ \wEtav{\xA} }

\def\weta{ \eta }
\def\wetav#1{ \weta^{\bar{#1}} }
\def\wetaa{ \wetav{\xa} }
\def\wetab{ \wetav{\xb} }

\def\wRho{ P }
\def\wRhov#1#2{ \wRho_{#1}^{#2} }
\def\wRhomA{ \wRhov{\xmu}{\xA} }

\def\wrho{ \rho }
\def\wrhov#1#2{ \wrho_{#1}^{#2} }
\def\wrhoma{ \wrhov{\xmu}{\xa} }

\def\wtheta{ \theta }
\def\wthetav#1{ \theta_{#1} }
\def\wthetaa{ \wthetav{\xa} }

\def\wF{ F }
\def\wFv#1{ \wF^{#1} }
\def\wFA{ \wFv{\xA} }

\def\wf{ f }
\def\wfnv#1{ \wf^{#1} }
\def\wfa{ \wfnv{\xa} }


==> defs/locdef1.tex <==
\def\aee{ $$ }
\def\aeee{ $$ }
\def\bee{ $ }
\def\beee{ $ }
\def\xlabel#1{ \nonumber }

\def\xId{ \mathbbm{1} }

\def\rnk{\mathop{\mathrm{rank}} }

\def\crvng{curving}
\def\crvngp{\crvng\ polynomial}

\def\ddf{divided difference}
\def\ddfs{\ddf s}

\def\ctL{ \mathsf{L} }
\def\ctLL{ \ddot{\ctL} }
\def\ctLLL{ \dddot{\ctL} }
\def\ctLLv#1{ \ctLL #1 }
\def\ctLLbv#1{ \ctLLv{(#1)} }
\def\ctLLXsom{ \ctLLv{\Xsom} }
\def\ctLLX{ \ctLLv{(\xX)} }
\def\ctLLTsU{ \ctLLbv{\TsxcA} }
\def\ctLLTsCn{ \ctLLbv{\Ts\IC^n} }

\def\ctLLTUS{ \ctLLv{ \mtdfTUS } }
\def\ctLLTUSk{ \ctLLv{ \mtdfTUSk } }
\def\ctLLTUh{ \ctLLv{ \mtdfTUh } }
\def\ctLLTYS{ \ctLLv{ \mtdfTYS } }

\def\qhlm{quasi-holomorphic}
\def\qhlmvb{\qhlm\ vector bundle}
\def\cqhlmvb{curved \qhlmvb}

\def\ctLLcrv#1#2{ \ctLL\brB{ (\xXv{#1},-\somv{#1})\times(\xXv{#2},\somv{#2}) } }
\def\ctLLcrot{ \ctLLcrv{1}{2} }

\def\ctLLXsomv#1{ \ctLL\Xsomv{#1} }
\def\ctLLXsomo{ \ctLLXsomv{1} }
\def\ctLLXsomt{ \ctLLXsomv{2} }

\def\xwd{well-defined}

\def\rmA{ \mathrm{A} }
\def\Ainf{ \rmA_\infty }
\def\tAinf{$\Ainf$}
\def\Ainfalg{\tAinf-algebra}
\def\fDAinfalg{filtered Dolbeault \Ainfalg}
\def\FDAi{FD\tAinf}
\def\cAinfalg{curved \Ainfalg}

\def\Khl{ K\"{a}hler }
\def\dR{de Rham}

\def\xpBd{`pseudo-Beltrami' differential}
\def\pBd{pseudo-Beltrami differential}

\def\xwk{weak}
\def\xacrv{curved}
\def\crtp{\xacrv\ 2-periodic}
\def\crtpc{\crtp\ category}

%\def\xrca{relative curved algebra}
%\def\tcrca{2-category of \xrca}

\def\xrca{relative curved differential graded polynomial algebra}
\def\tcrca{2-category of \xrca s}
\def\yCDG{CDG}




\def\smcl{semi-classical}
\def\smclgrd{\smcl\ grading}
\def\smcldgr{\smcl\ degree}

\def\xrl{relative}
\def\xrlb{relatively balanced}
\def\xrlnn{relatively non-negative}

\def\Dlb{Dolbeault}
\def\Dlbf{\Dlb\ filtration}
\def\DGA{DGA}
\def\DDGA{DDGA}
\def\hK{hyper-\K}
\def\K{K\"{a}hler}
\def\Knr{Knorrer}
\def\Knrp{\Knr\ periodicity}

\def\blncd{balanced}
\def\blncdv#1{$#1$-\blncd}
\def\blncdn{\blncdv{n}}
\def\blncdt{\blncdv{2}}
\def\blncdh{\blncdv{3}}
\def\blncdz{\blncdv{0}}

\def\NSb{Schouten–-Nijenhuis bracket}

\def\CM{Maurer-Cartan}
\def\CMe{\CM\ equation}
\def\CMlt{\CM\ element}

\def\Ldr{Legendre}
\def\Ldrt{\Ldr\ transform}

\def\ooc{$(1,1)$-curvature}

\def\xPoi{Poisson}
\def\xGrs{Gerstenhaber}
\def\xLie{Lie}
\def\DLa{differential \xLie\ algebra}
\def\DPa{differential \xPoi\ algebra}
\def\DGa{differential \xGrs\ algebra}
\def\PGa{\xPoi-\xGrs\ algebra}
\def\PGa{\xLie-\xGrs\ algebra}
\def\DPGa{differential \PGa}

\def\rlcn{relative connection}
\def\darc{\DLa\ of \rlcn s}

\def\pgbvv#1#2{ [ #1,#2 ]_{\rm LG } }
\def\pgbdd{ \pgbvv{\cdot}{\cdot} }

\def\pgD{ D }
\def\pgDv#1{ \pgD_{#1} }
\def\pgDa{ \pgDv{\pga} }

\def\pga{ \alpha }
\def\pgae{ \dfev{\pga} }
\def\pgav#1{ \pga_{|#1} }
\def\pgai{ \pgav{i} }
\def\pgao{ \pgav{1} }
\def\pgat{ \pgav{2} }
%\def\pgb{ \beta }
\def\xpgv#1{ \tilde{#1} }
%\def\pgb{ \xpgv{\alpha} }
\def\pgb{ \phi }
%\def\pgdg{ b }
\def\pgdg{ d_{[\;]} }

\def\zdpa{ \mathscr{P} }
\def\zdpaXsom{ \zdpa\Xsom }
\def\zdpaTsU{ \zdpa(\TsU) }
\def\zdpaT{ \zdpa_{\Ts} }
\def\zdpaTv#1{ \zdpaT(#1) }
\def\zdpaTU{ \zdpaTv{\xcA} }

\def\zdga{ \mathscr{G} }
\def\zdgav#1{ \zdga(#1) }
\def\zdgaU{ \zdgav{\xcA} }
\def\zdgalv#1{ \zdga_{#1} }
\def\zdgalW{ \zdgalv{\xcW} }
\def\zdgalWU{ \zdgalW(\xcA) }
\def\zdgalWotU{ \zdgalv{\xcWot}(\xcA) }

\def\zdrc{ \mathscr{C} }
\def\zdrcEnb{ \zdrc\adgmE }

\def\cdlv#1{ [#1] }
\def\cdlv#1{ \check{#1} }
\def\cpgao{ \cdlv{\pga}_{|1} }

\def\Dhbvf{\Dlb\ holomorphic bi-vector field}

\def\inftsm{infinitesimal}
\def\inftsmly{infinitesmilally}

\def\tKmf{Koszul matrix factorization}
\def\tKc{Koszul complex}


\def\xtran{2-translation}
\def\ytran{2-translation}

\def\Mlc{Micro-local}
\def\mlc{micro-local}
\def\mlcz{micro-localization}
\def\prshf{presheaf}
\def\mlcs{\mlc\ \prshf}



\def\zCtng{Cotangent}
\def\zCtngr{\zCtng\ version}
\def\zctng{cotangent}
\def\zctngr{\zctng\ version}
\def\zctngb{\zctng\ bundle}
\def\zdctngb{deformed \zctngb}

\def\zAffn{Affine}
\def\zAffnr{\zAffn\ version}
\def\zaffn{affine}
\def\zaffnr{\zaffn\ version}

\def\zsaff{symplectic \zaffn}

\def\Sd{Self-dual}
\def\Sdb{\Sd\ bundle}
\def\sd{self-dual}
\def\sdb{\sd\ bundle}


\def\xrD{ \mathrm{D} }
\def\stp{ 2 -\mathrm{p} }
\def\rD{ \xrD_{\stp} }
\def\rb{ \mathrm{b} }
\def\rDb{ \xrDs^\rb }
%\def\prftpv#1{ #1^{\mathrm{prf}}_{\xmtp} }
\def\prftpv#1{ #1_{\Zt} }
%\def\prftpv#1{ #1^2 }
%\def\prftapv#1{ #1^{\mathrm{prf,aug}}_{\xmtp} }
%\def\prftapv#1{ #1^{\mathrm{aug}}_{\Zt} }
\def\prftapv#1{ #1^{\mathrm{a}}_{\Zt} }
\def\rDprf{ \prftpv{\xrDs} } %^{\mathrm{prf}}_{\xmtp} }
\def\rDprfa{ \prftapv{\xrDs} }
%\def\rDDprf{ \prftpv{\drD} }
\def\rDprftp{ \rDprf_{2-\mathrm{p}} }
\def\rDprfbv#1{ \rDprf #1  }
\def\rDprfbA{ \rDprfbv{\ycdgaA} }

\def\rDprfcA{ \rDprf(\xdlA) }
\def\rDprfcAdv#1{ \rDprfcA\ctrnv{#1} }
\def\rDprfcAdn{ \rDprfcAdv{n} }
\def\rDprfcAdo{ \rDprfcAdv{1} }
\def\rDprfcAAbx{ \rDprf(\xdlA\otimes\xdlAbx) }

\def\rDprfU{ \rDprf(\xcA) }

\def\xrDs{ \mathsf{D} }
\def\xrDsd{ \ddot{\xrDs} }
\def\xrDsdd{ \dddot{\xrDs} }
\def\rDsprf{ \prftpv{\xrDs} }
\def\rDDprf{ \prftpv{\xrDsd} }
\def\rDDDprf{ \prftpv{\xrDsdd} }
\def\rDDprfv#1{ \rDDprf(#1) }
\def\rDDprfU{ \rDDprf(\xcA) }
%\def\rDDprfUxVy{ \rDDprf(\UxVy) }
\def\rDDprfUxVy{ \ctLLv(\UxVy) }
%\def\rDDprfaUxVy{ \rDDprfa(\UxVy) }
\def\rDDprfaUxVy{ \ctLLv(\UxVy) }
%\def\rDDprfaUxVypp{ \rDDprfa(\UxVypp) }
\def\rDDprfaUxVypp{ \ctLLv(\UxVypp) }
%\def\rDDprfaUpxVy{ \rDDprfa(\UpxVy) }
\def\rDDprfaUpxVy{ \ctLLv(\UpxVy) }
%\def\rDDprfaVyUx{ \rDDprfa(\VyUx) }
\def\rDDprfaVyUx{ \ctLLv(\VyUx) }

%\def\rDDprfaVmyUx{ \rDDprfa(\VmyUx) }
\def\rDDprfaVmyUx{ \ctLLv(\VmyUx) }
%\def\rDDprfaVyUmx{ \rDDprfa(\VyUmx) }
\def\rDDprfaVyUmx{ \ctLLv(\VyUmx) }

\def\rDDprfUS{ \rDDprf(\xcA,\xsfS) }
\def\rDDprfUSk{ \rDDprf(\xcA,\hdf) }
\def\rDDprfYoSk{ \rDDprf(\yYo,\hdf) }
\def\rDDprfUSek{ \rDDprf(\xcA,\dfe\hdf) }
%\def\rDDprfUSe{ \rDDprf(\xcA,\xsfSe) }
\def\rDDprfUSe{ \rDDprf(\xcA,\dfe\xsfS) }
\def\rDDprfUhe{ \rDDprf(\xcA,\hdfe) }
\def\rDDprfUhae{ \rDDprf(\xcA,\ehdf) }
\def\rDDprfUp{ \rDDprf(\xcAp) }
\def\rDDprfY{ \rDDprf(\yY) }
\def\rDDprfYS{ \rDDprf(\yY,\ysfSY) }
\def\rDprfY{ \rDprf(\yY) }
\def\rDprfX{ \rDprf(\xX) }

\def\rDsprfa{ \prftapv{\xrDs} }
\def\rDDprfa{ \prftapv{\xrDsd} }
\def\rDDDprfa{ \prftapv{\xrDsdd} }
\def\rDDprfav#1{ \rDDprfa(#1) }
\def\rDDprfaU{ \rDDprfa(\xcA) }
\def\rDDprfaUS{ \rDDprfa(\xcA,\xsfS) }
\def\rDDprfaUh{ \rDDprfa(\xcA,\hdf) }
\def\rDDprfaUp{ \rDDprfa(\xcAp) }

\def\rDprfvv#1#2{ \rDprf(#1,#2) }
\def\rDprfBvv#1#2{ \rDprf\Big(#1,#2\Big) }
\def\rDprfUW{ \rDprfvv{\xcA}{\xcW} }
\def\rDprfUWv#1{ \rDprfvv{\xcAv{#1}}{\xcWv{#1}} }
\def\rDprfUWo{ \rDprfUWv{1} }
\def\rDprfUWt{ \rDprfUWv{2} }

\def\rDprfcUWv#1{ \rDprfvv{\xcUv{#1}}{\xcWv{#1}} }
\def\rDprfcUWo{ \rDprfcUWv{1} }
\def\rDprfcUWt{ \rDprfcUWv{2} }

\def\rDsprfv#1{ \rDsprf(#1) }
\def\rDsprfU{ \rDsprfv{\xcA} }
\def\rDsprfY{ \rDsprfv{\yY} }
\def\rDsprfYot{ \rDsprfv{\yYot} }
\def\rDsprfcYoct{ \rDsprfv{\ycYoct} }

\def\rDsprfvv#1#2{ \rDsprf(#1,#2) }
\def\rDsprfsvv#1#2{ \rDsprf(#1;#2) }
\def\rDsprfavv#1#2{ \rDsprfa(#1,#2) }
\def\rDsprfBvv#1#2{ \rDsprf\Big(#1,#2\Big) }
\def\rDsprfbvv#1#2{ \rDsprf\big(#1,#2\big) }
\def\rDsprfUW{ \rDsprfvv{\xcA}{\xcW} }
\def\rDsprfUWtmo{ \rDsprfvv{\xcA}{\xcWt-\xcWo} }
%\def\rDsprfUWot{ \rDsprfvv{\xcA}{\xcWot} }
\def\rDsprfUba{ \rDsprfsvv{\xcA}{\xmmbf} }
%\def\rDsprfUWd{ \rDsprfUW_{\cdfm} }
\def\rDsprfUWd{ \rDsprfvv{\xcA}{\xcW;\xdfm} }
\def\rDsprfUd{ \rDsprfvv{\xcA}{\xdfm} }
\def\rDsprfUdot{ \rDsprfsvv{\xcA}{\xdfmot} }
\def\rDsprfYdot{ \rDsprfsvv{\yYot}{\xdfmot} }
%\def\rDsprfYxdot{ \rDsprfsvv{\ycYo \ycapX \ycYt}{\xdfmot} }
\def\rDsprfYxdot{ \rDsprfsvv{\ycYoct}{\xdfmot} }
\def\rDsprfYxdoct{ \rDsprfsvv{\yYoct}{\xdfmot} }
\def\rDsprfYadoct{ \rDsprfsvv{\yYoct}{\adfmot} }
\def\rDsprfYoxdoct{ \rDsprfsvv{\yYo}{\xdfmot} }
\def\rDsprfUWde{ \rDsprfvv{\xcA}{\xcW;\xdfme} }
\def\rDsprfUeWot{ \rDsprfvv{\xcAekot}{\xcWot} }
\def\rDsprfUeWoh{ \rDsprfvv{\xcAekoh}{\xcWoh} }
\def\rDsprfUeWth{ \rDsprfvv{\xcAekth}{\xcWth} }
\def\rDsprfUWz{ \rDsprfvv{\xcA}{\xcWz} }
\def\rDsprfUmW{ \rDsprfvv{\dfmU}{\xcWe} }
\def\rDsprfYlY{ \rDsprfvv{\yY}{\xdfmY} }

\def\rDsprfUmWv#1{ \rDsprfvv{\dfmUmv{#1}}{\xcWve{#1}} }
\def\rDsprfUmWot{ \rDsprfUmWv{12} }
\def\rDsprfUmWth{ \rDsprfUmWv{23} }
\def\rDsprfUmWoh{ \rDsprfUmWv{13} }

\def\rDsprfUWav#1{ \rDsprfvv{\xcA}{\xcWv{#1}} }
\def\rDsprfUWao{ \rDsprfUWav{1} }
\def\rDsprfUWat{ \rDsprfUWav{2} }
\def\rDsprfaUW{ \rDsprfavv{\xcA}{\xcW} }
\def\rDsprfaUWot{ \rDsprfavv{\xcA}{\xcWot} }
\def\rDsprfUWv#1{ \rDsprfvv{\xcAv{#1}}{\xcWv{#1}} }
\def\rDsprfUWo{ \rDsprfUWv{1} }
\def\rDsprfUWt{ \rDsprfUWv{2} }
\def\rDsprfUWot{ \rDsprfUWav{12} }
\def\rDsprfLWQ{ \rDsprfvv{\vcL}{\xcW + \xcWq} }
%\def\rDsprfmvv#1#2#3{ \rDsprf\lrbc{#1,#2;#3} }
\def\rDsprfmvv#1#2#3{ \rDsprfvv{#1}{#2}\ytrnv{#3} }
\def\rDsprfamsvv#1#2{ \rDsprfa\lrbc{#1;#2} }
\def\rDsprfmsvv#1#2{ \rDsprf\lrbc{#1;#2} }
\def\rDsprfamvv#1#2#3{ \rDsprfa\lrbc{#1,#2;#3} }
\def\rDsprfmUWL{ \rDsprfmvv{\xcA}{\xcW}{\vcL} }
%\def\rDsprfmv#1#2{ \rDsprf(#1;#2) }
\def\rDsprfmv#1#2{ \rDsprf(#1)\ytrnv{#2} }

\def\dccs{derived category of coherent sheaves}
\def\Fk{Fukaya}
\def\FkF{\Fk-Floer}
\def\FkFc{\FkF\ category}
%\def\rFuk{ \mathrm{Fuk} }
\def\rFuk{ \mathrm{F} }
\def\rCoh{ \mathrm{Coh} }
\def\TQFT{TQFT}

\def\pb{pull-back}
\def\pf{push-forward}
\def\ccm{curved complex manifold}

\def\tqft{topological quantum field theory}
\def\tqfts{topological quantum field theories}

\def\lgr{lagrangian}
%\def\hlgr{holomorphic \lgr}
\def\hlgr{\lgr}
\def\hlgrsm{\hlgr\ submanifold}
\def\hlsm{holomorphic symplectic}
\def\hlsmf{\hlsm\ form}
\def\hlsmm{\hlsm\ manifold}
\def\hlsms{\hlsm\ structure}
\def\fCY{Calabi-Yau}
\def\fsCY{CY}
\def\hsCY{half-\fsCY}
\def\fcp{complex}
\def\lgfbr{\lgr\ fibration}
\def\hlgfbr{holomorphic \lgfbr}



\def\gnfn{generating function}
\def\gnfns{\gnfn s}

\def\tpd{2-periodic}
\def\xmtp{ 2-\mathrm{p} }

\def\tpdpr{\tpd\ \xper}
\def\tpdprc{\tpdpr\ category}

\def\dccs{derived category of coherent sheaves}
\def\bdccs{bounded \dccs}
\def\tpdccs{2-periodic \dccs}
\def\tpcmp{2-periodic complex}
\def\tpcmpsh{\tpcmp\ of sheaves}
\def\fwlb{fibration over a lagrangian base}
\def\fwlbs{fibrations over lagrangian bases}
\def\fwwlbs{fibrations with lagrangianl bases}
\def\cfwwlbs{category of \fwwlbs}
\def\hfwlbs{holomorphic \fwlbs}
\def\hfwlb{holomorphic \fwlb}

\def\hlfb{holomorphic fibration}
\def\fbl{fiber bundle}

\def\ah{anti-holomorphic}
\def\xah{$(0,\bullet)$}
\def\xahf{\xah-form}
\def\xahfs{\xahf s}

\def\cDla{CDlA}

\def\xau{augment}
\def\xaug{augmented}
\def\xAug{Augmented}
\def\xaugm{augmentation}

\def\xalg{algebraic}
\def\pdcat{perfect derived category}
\def\Ztpdcat{\tpd\ \pdcat}
\def\ZtPDC{$\Zt$-PDC}
\def\cdga{curved differential graded algebra}
\def\CDGA{CDGA}
\def\dgm{differential graded module}
\def\Ztdgm{\Ztgrdd\ differential  module}
%\def\Ztdgm{\Ztgrdd\ module}
\def\DGM{DGM}
\def\DGM{GDM}
\def\ZtDGM{$\Zt$-\DGM}

\def\gfn{generating function}

\def\sffc{second fundamental form class}
\def\SFFC{SFFC}

\def\corr{correspondence}
\def\corrs{\corr s}
\def\hlcorr{holomorphic correspondence}
\def\hlgcorr{\hlgr\ correspondence}

\def\xxtf{2-functor}
\def\cfun{correspondence \xxtf}
\def\Ltf{Legendre \xxtf}

\def\hlfcorr{holomorphic fibration correspondence}
\def\hlgfcorr{\hlgr\ fibration correspondence}

\def\lgcr{lagrangian correspondence}
\def\lgcrf{\lgcr\ functor}

%\def\dztgrm{differential \Ztgrdd\ module}
\def\dztgrm{\Ztgrdd\ module}
%\def\DGM{DGM}
\def\DGMs{\DGM s}
\def\pDGM{\xper\ \DGM}

\def\xper{perfect}
\def\xprm{\xper\ module}
\def\xprmi{\xprm}
\def\xprms{\xprm s}

\def\Ac{Atiyah class}
\def\cAc{curved \Ac}

\def\xad{admissible}
%\def\xad{resolvable}
\def\xadm{\xad\ module}
\def\xadms{\xadm s}

\def\FM{Fourier-Mukai}
\def\FMtr{\FM\ transform}
\def\FMtrs{\FMtr s}

\def\opfib{1-point fibration}
\def\copfib{curved \opfib}

\def\spmnf{special manifold}
\def\spmp{special map}

\def\xfp{fiber-product}
\def\fbcr{fiber-critical}
\def\xsprt{support}
\def\xep{embedding-projection}
\def\xeps{\xep s}

%\def\cfb{curved fibration}
\def\cfb{curved complex manifold}
\def\cfbs{\cfb s}
\def\xcfb{curved fibration}
\def\xcfbs{\xcfb s}

\def\xempt{identity}
\def\xempto{\xempt\ object}

\def\rmon{rigid monoidal}
\def\rmonNc{\rmon\ $\zN$-category}

\def\idend{identity endomorphism}

\def\psmon{pseudo-monoidal}

\def\xgd{clean}
\def\gdint{\xgd\ intersection}
\def\ygd{\xgd}

\def\zord{order}

\def\xanl{analytic }

\def\xstr{structure}
%\def\dstrv#1{#1-dimensional structure}
\def\dstrv#1{#1-structure}
\def\thstr{\dstrv{3}}
\def\tstr{\dstrv{2}}
\def\ostr{\dstrv{1}}
\def\zstr{\dstrv{0}}
\def\nstr{\dstrv{n}}
\def\nmostr{\dstrv{$(\zn-1)$}}
\def\nmtstr{\dstrv{$(\zn-2)$}}
\def\npostr{\dstrv{$(\zn+1)$}}
\def\Nstr{\dstrv{N}}

\def\trsp{transparent}
\def\trsp{invisible}
\def\trsply{invisibly}

\def\zN{ d }
\def\zn{ n }

\def\dsu{disjoint union}
\def\dsuf{\dsu\ functor}
\def\glu{gluing}
\def\gluf{\glu\ functor}

\def\xmf{matrix factorization}
\def\xmfs{\xmf s}
\def\cxmf{category of \xmf}
\def\xgmf{global \xmf}
\def\xgmfs{\xgmf s}
\def\tZtgdcs{\tpd\ category of a \cfb}

\def\cDA{curved Dolbeault algebra}



\def\cnjg{conjugate}
\def\cnjgd{\cnjg\ decorated}

\def\pgluf{ \# }
\def\xgluf{ \xobv{\pgluf} }
%\def\xobgluf{ \xobv{\xgluf} }

\def\pglufv#1{ \pgluf_{#1} }
\def\pglufbvv#1#2{ \pglufv{#1}\big(#2\big) }
\def\xobpglufv#1{ \xobwv{\pglufv{#1}} }
\def\xobpglufstMn{ \xobpglufv{\stMn} }


\def\ocng#1{ \bar{#1} }
\def\ocngw#1{ \overline{#1} }

\def\Amdl{$A$-model}
\def\Amdls{\Amdl s}
\def\Bmdl{$B$-model}
\def\Bmdls{\Bmdl s}

\def\tgsp{target space}
\def\sgmd{sigma-model}
\def\sgmds{\sgmd s}
%\def\tsgmd{topological \sgmd}
\def\tsgmd{TSM}
\def\thsgmd{3-dimensional \tsgmd}

\def\TQFTf{\TQFT\ functor}

\def\ctps{cut and paste}
\def\ctpst{\ctps\ topology}
\def\CWc{$CW$-complex}
\def\Wln{Wilson line}
\def\Wlns{\Wln s}

\def\Sdual{Serre-dual}

\def\idfib{identity fibration}

\def\crvng{curving}
\def\crvngs{\crvng s}


\def\xctg{category}
\def\xactg{a \xctg}

\def\xX{ X }
\def\xXv#1{ \xX_{#1}}
\def\xXo{ \xXv{1} }
\def\xXt{ \xXv{2} }
\def\xXh{ \xXv{3} }
\def\xXf{ \xXv{4} }
\def\tX{ \tilde{\xX} }
\def\xXp{ \xX\p }
\def\xZ{ Z }
\def\xSg{ \Sigma }
\def\bSg{ \bar{\xSg} }
\def\ySg{ S }
\def\xSgb{ \xSg_{\mathrm{b}} }
\def\xSgbp{ \xSg_{\mathrm{b}}\p }
\def\xM{ M }
\def\xMp{ \xM\p }
\def\xL{ L }
\def\xLpl{ \xL_+ }
\def\xLpls{ \xLpl^{\udl} }
\def\xC{ C }
\def\xI{ I }
\def\xP{ P }
\def\xPp{ \xP\p }

\def\Tng{ \mathrm{T} }
%\def\Ts{ \Tng^\ast }
\def\Ts{ \Tvs }
\def\bTng{ \bar{\Tng} }
%\def\bTs{ \bTng^\ast }
\def\bTs{ \dulv{\bTng} }
\def\Tsv#1{ \Ts #1 }

\def\TsU{ \Tsv{\xcA} }
\def\TsUz{ \Tsv{\xcAz} }
\def\TscU{ \Tsv{\xcU} }

\def\TsUdf{ (\TsU)_{\xsfS} }

\def\Tngv#1{ \Tng #1 }


\def\xcU{ \mathcal{U} }
\def\xcUp{ \xcU\p }
\def\xcUv#1{ \xcU_{#1} }
\def\xcUo{ \xcUv{1} }
\def\xcUt{ \xcUv{2} }
\def\xcUh{ \xcUv{3} }
\def\xcUot{ \xcUv{12} }
\def\xcUth{ \xcUv{23} }
\def\xcUhf{ \xcUv{34} }

\def\TxcA{ \Tng\xcA }
\def\TsxcA{ \Ts\xcA }

\def\Nrm{ \mathrm{N} }

\def\Vfb{ V }
\def\Vfbv#1{ \Vfb_{#1} }
\def\Vfbx{ \Vfbv{x} }
\def\xcA{ U }
\def\xcAp{ \xcA\p }
\def\xcAv#1{ \xcA_{#1} }
\def\xcAz{ \xcAv{0} }
\def\xcAo{ \xcAv{1} }
\def\xcAt{ \xcAv{2} }
\def\xcAh{ \xcAv{3} }
\def\xcAf{ \xcAv{4} }
\def\TsA{ \Tsv{\xcA} }
\def\xcV{ V }
\def\xcVp{ \xcV\p }
\def\xcVv#1{ \xcV_{#1} }
\def\xcVo{ \xcVv{1} }
\def\xcVot{ \xcVv{12} }
\def\xcVt{ \xcVv{2} }
\def\xcVh{ \xcVv{3} }
\def\xfbv#1{ #1_{\mathrm{fbr}} }
\def\xfbnv#1#2{ #1_{\mathrm{fbr},#2} }
%\def\Vfb{ \xfbv{\xcV} }
%\def\Vfbv#1{ \xfbnv{\xcV}{#1} }
\def\Vfbo{ \Vfbv{1} }
\def\Vfbt{ \Vfbv{2} }

\def\xcrtv#1#2{ #1_{#2} }
\def\xcAWz{ \xcrtv{\xcA}{\xcWz} }
\def\xcAW{ \xcrtv{\xcA}{\xcW} }
\def\xcAWot{ \xcrtv{\xcA}{\xcWot} }
\def\crWbsot{ \xcrtv{\xcA}{\DlWbs} } % {\xcWbst-\xcWbso} }

\def\ycA{ A }
\def\ycb{ \beta }

\def\xtwD{ D }
\def\txtwD{ \tilde{ \xtwD } }
\def\xtwDv#1{ \xtwD_{#1} }
\def\xtwDE{ \xtwDv{\xE} }

%\def\xcW{ \mathcal{W} }
\def\xcW{ W }
\def\xtt{\mathrm{tot}}
\def\xcWtt{\xcW^{\xtt} }
\def\xcWtthx{\xcWtt_{\mathrm{hex}} }
\def\xcWttrc{\xcWtt_{\mathrm{rect}} }
\def\xcWttrcv#1{ \xcWtt_{\mathrm{rect},#1} }
\def\xcWttrcot{ \xcWttrcv{12} }
\def\xcWttrcto{ \xcWttrcv{21} }
\def\xcWttv#1{ \xcWtt_{#1} }
\def\xcWttt{ \xcWttv{2} }
\def\xcWttot{ \xcWttv{12} }
\def\xcWp{ \xcW\p }
\def\xcWv#1{ \xcW_{#1} }
\def\xcWo{ \xcWv{1} }
\def\xcWi{ \xcWv{i} }
\def\xcWot{ \xcWv{12} }
\def\xcWoh{ \xcWv{13} }
\def\xcWth{ \xcWv{23} }
\def\xcWbs{ \xcW_{\mathrm{bs}} }
\def\xcWbsv#1{ \xcW_{\mathrm{bs},#1} }
\def\xcWbso{ \xcWbsv{1} }
\def\xcWbst{ \xcWbsv{2} }
\def\xcWop{ \xcWo\p }
\def\xcWop{ \widetilde{\xcWo} }
\def\xcWt{ \xcWv{2} }
\def\xcWh{ \xcWv{3} }
\def\xcWot{ \xcWv{12} }
\def\xcWth{ \xcWv{23} }
\def\xcWz{ \xcW_{0} }
\def\xcWpl{ \xcW_{+} }
\def\xE{ E }
\def\xEs{ \xE^\ast }
\def\xEv#1{ \xE^{#1} }
\def\xEdv#1{ \xE_{#1} }
\def\xEo{ \xEdv{1} }
\def\xEt{ \xEdv{2} }
\def\xEh{ \xEdv{3} }
\def\xEi{ \xEdv{i} }
\def\xEot{ \xEdv{12} }
\def\xEpot{ \xEot\p }
\def\xEth{ \xEdv{23} }
\def\xEpth{ \xEth\p }
\def\xEoh{ \xEdv{13} }
\def\xEev{ \xEv{\yev} }
\def\xEod{ \xEv{\yod} }
\def\xEp{ \xE\p }
\def\xD{ D }
\def\xDv#1{ \xD_{#1} }
\def\xDE{ \xDv{\xE} }

\def\scE{ \mathscr{E} }
\def\scEv#1{ \scE_{#1} }
\def\scEo{ \scEv{1} }
\def\scEt{ \scEv{2} }
\def\scO{ \mathscr{O} }
\def\strs#1{ \scO_{#1} }
\def\strsU{ \strs{\xcA} }
\def\strsY{ \strs{\yY} }
\def\strsYo{ \strs{\yYo} }
\def\strsYt{ \strs{\yYt} }

\def\xcp{ p }
\def\xcpv#1{ \xcp_{#1} }
\def\xcpo{ \xcpv{1} }
\def\xcpt{ \xcpv{2} }
\def\xcpot{ \xcpv{12} }

\def\xcF{ F }
\def\xcFv#1{ \xcF_{#1} }
\def\xcFot{ \xcFv{12} }
\def\xcFth{ \xcFv{23} }

\def\xcE{ \cE }
\def\xcEv#1{ \xcE_{#1} }
\def\xcEo{ \xcEv{1} }
\def\xcEt{ \xcEv{2} }
\def\xcEot{ \xcEv{12} }
\def\xcEotp{ \xcEot\p }
\def\xcEth{ \xcEv{23} }
\def\xcEoh{ \xcEv{13} }

\def\xHomv#1#2{ \Hom(#1,#2) }
\def\xHomEEp{ \xHomv{\xE}{\xEp} }
\def\xbOm{ {\Omega} }
\def\xbOmxvv#1#2{ \xbOm^{#1,#2} }
\def\xbOmxzv#1{ \xbOmxvv{0}{#1} }
\def\xbOmxvb#1{ \xbOmxvv{#1}{\bullet} }
\def\xbOmxve#1{ \xbOmxvv{#1}{\yev} }
\def\xbOmxvo#1{ \xbOmxvv{#1}{\yod} }
\def\xbOmxvb#1{ \xbOmxvv{#1}{\bullet} }
\def\xbOmoe{ \xbOmxve{1} }
\def\xbOmoo{ \xbOmxvo{1} }
\def\xbOmbe{ \xbOmxvb{1} }
\def\xbOmbz{ \xbOmxvb{0} }
\def\xbOmv#1{ \xbOm^{0,#1} }
%\def\xbOmv#1{ \xbOmvv{0}{#1} }
\def\xbOmz{ \xbOmv{0} }
\def\xbOmb{ \xbOmv{\bullet} }
\def\xbOme{ \xbOmv{\yev} }
\def\xbOmev#1{ \xbOme(#1) }
\def\xbOmeU{ \xbOmev{\xcA} }
\def\xbOmeEE{ \xbOmev{\End\xE} }
\def\xbOmecU{ \xbOmev{\xcU} }
\def\xbOmecUp{ \xbOmev{\xcUp} }
\def\xbOmo{ \xbOmv{\yod} }
\def\xbOmov#1{ \xbOmo(#1) }
\def\xbOmbv#1{ \xbOmb(#1) }
\def\xbOmBv#1{ \xbOmb\big(#1\big) }
\def\xbOmbE{ \xbOmbv{\xE} }
\def\xbOmbeE{ \xbOmBv{\End(\xE) } }
\def\xbOmbzeE{ \xbOmBv{\End\xE } }

\def\xbOmbX{ \xbOmbv{\xX} }
\def\xbOmbU{ \xbOmbv{\xcA} }
\def\xbOmbUp{ \xbOmbv{\xcAp} }
\def\xbOmbEEp{ \xbOmb\big( \xHomEEp\big) }
\def\xbOmbU{ \xbOmbv{\xcA} }

\def\xbOmvv#1#2{ \xbOmv{#1}\lrbc{#2} }
\def\xbOmEv#1{ \xbOmvv{#1}{\xE} }
\def\xbOmevE{ \xbOmEv{\yev} }
\def\xbOmodE{ \xbOmEv{\yod} }
\def\xbOmodev#1{ \xbOmv{\yod} \brb{\End(#1)} }
\def\xbOmodeE{ \xbOmodev{\xE} }

\def\xbOmov#1{ \xbOmvv{1}{#1} }
\def\xbOmoU{ \xbOmov{\xcA} }

\def\xbOmbUUST{ \xbOmbv{\xcA,\SbTU} }
\def\xbOmoUUST{ \xbOmov{\xcA,\SbTU} }
\def\xbOmbX{ \xbOmbv{\xX} }
\def\xbOmbUST{ \xbOmbv{\TsU} }

\def\xbOmbUUWT{ \xbOmbv{\xcA,\WbTU} }
\def\xbOmeUUWT{ \xbOmev{\xcA,\WbTU} }

\def\xbOmzv#1{ \xbOmvv{0}{#1} }
%\def\xbOmxov#1{ \xbOmvv{1}{#1} }
\def\xbOmxob{ \xbOmxvb{1} }


\def\xbOmoeE{ \xbOmoe\brb{\End \xE} }
\def\xbOmooE{ \xbOmoo\brb{\End \xE} }

\def\xbOmbeE{ \xbOmbe\brb{\End \xE} }

\def\xbOmoeEoh{ \xbOmoe\brb{\End \xEoh} }

\def\xMia{ \xM_{i,\alpha} }
\def\xMimoa{ \xM_{i-1,\alpha} }

\def\yW{ W }
\def\ycW{ \mathcal{\yW} }
\def\yU{ U }

\def\xXcv#1{ \xX^{\times #1} }
\def\xXcn{ \xXcv{n} }
\def\xXcnt{ \xXcv{(n+2)} }

\def\rDbv#1{ \rD\big( #1 \big) }
\def\rDv#1{ \rD(#1) }
\def\rDBv#1{ \rD\Big(#1\Big) }
\def\rDbv#1{ \rD\big(#1\big) }
%\def\rDX{ \rDv{\xX} }
\def\rDX{ \rDv{\xcA} }
\def\rDXp{ \rDv{\xXp} }
\def\rDW{ \rDv{\ycW} }

\def\xrDbv#1{ \xrD\big( #1 \big) }
\def\xrDv#1{ \xrDs^{\mathrm{b}}(#1) }
\def\xrDX{ \xrDv{\xX} }

\def\xN{ N }
\def\xNp{ \xN\p }

%\def\rDX{ \rD(\xX) }


\def\Sodv#1{ (S^1)^{\sqcup #1} }
\def\Sodn{ \Sodv{n} }
\def\Sodnt{ \Sodv{(n+2)} }

\def\Idv#1{ I^{\sqcup #1} }
\def\Idm{ \Idv{m} }

\def\cX{ \mathcal{X} }
\def\cXv#1{ \cX\lrbc{#1} }
\def\cXbv#1{ \cX\big(#1\big) }
\def\cXSodn{ \cXbv{\Sodn} }
\def\cXN{ \cXv{\xN} }

\def\ccX{ \mathcal{X} }
\def\ccXv#1{ \ccX\lrbc{#1} }
\def\ccXbv#1{ \ccX\big(#1\big) }
\def\ccXP{ \ccXv{\xP} }
\def\ccXPp{ \ccXv{\xPp} }
\def\ccXMz{ \ccXv{\stMz} }

\def\xcD{ \mathcal{D} }

\def\cC{ \mathcal{C} }
\def\cCv#1{ \cC\lrbc{#1} }
\def\cCbv#1{ \cC\big(#1\big) }
\def\cCN{ \cCbv{\xN} }
\def\cCSodn{ \cCbv{\Sodn} }

\def\cCmv#1{ \cC^{#1} }
\def\cCmN{ \cCmv{\zN} }
\def\cCmNv#1{ \cCmN_{#1} }
\def\cCmNi{ \cCmNv{i} }
\def\cCmNimo{ \cCmNv{i-1} }
\def\cCmNN{ \cCmNv{\zN} }
\def\cCmh{ \cCmv{3} }

\def\ccC{ \cC\!\!\cC }
\def\ccCv#1{ \ccC\lrbc{#1} }
\def\ccCbv#1{ \ccC\big(#1\big) }
\def\ccCP{ \ccCv{\xP} }

\def\xp{ p }
\def\shfv#1{ \mathscr{#1} }
\def\mdfv#1{ \mathcal{#1} }
\def\cE{ \mdfv{E} }
\def\cEs{ \cE^\ast }
\def\cEv#1{ \cE_{#1} }
\def\cEo{ \cEv{1} }
\def\cEt{ \cEv{2} }
\def\cEh{ \cEv{3} }
\def\cEp{ \cEv{\xp} }
\def\cEl{ \cEv{\xl} }
\def\cEb{ \cEv{\bullet} }

\def\cEot{ \cEv{12} }
\def\cEth{ \cEv{23} }

\def\cM{ \mdfv{M} }
\def\cP{ \mdfv{P} }
\def\cPp{ \cP\p }
\def\cPv#1{ \cP_{#1} }
\def\cPo{ \cPv{1} }
\def\cPt{ \cPv{2} }

\def\cM{ \mdfv{M} }
\def\cMp{ \cM\p }
\def\cMv#1{ \cM_{#1} }
\def\cMo{ \cMv{1} }
\def\cMt{ \cMv{2} }

\def\cfM{ \mdfv{M} }
\def\cfMp{ \cfM\p }
\def\cfMv#1{ \cfM_{#1} }
\def\cfMo{ \cfMv{1} }
\def\cfMt{ \cfMv{2} }
\def\cfMot{ \cfMv{12} }
\def\cfMth{ \cfMv{23} }
\def\cfMoh{ \cfMv{13} }
\def\cfMyot{ \cfMv{\ayo,\ayt} }

\def\cP{ \mdfv{P} }
\def\cPp{ \cP\p }

\def\cW{ \mdfv{W} }
\def\cWv#1{ \cW^{#1} }
\def\cWv#1{ \xvprvv{#1}{\xcW} }
\def\cWvv#1#2{ \cWv{\,#1}_{\,#2} }
\def\cWvv#1#2{ \xvprvv{#1}{\xcWv{#2} } }
\def\cWx{ \cWv{\bax} }
\def\cWy{ \cWv{\bay} }
\def\cWz{ \cWv{\baz} }
\def\cWu{ \cWv{\bau} }
\def\cWe{ \cWv{\varnothing} }
\def\cWa{ \cWv{\baa} }

\def\cWxo{ \cWvv{\bax}{1} }
\def\cWyt{ \cWvv{\bay}{2} }
\def\cWzh{ \cWvv{\baz}{3} }

\def\cWyo{ \cWvv{\bay}{1} }
\def\cWzt{ \cWvv{\baz}{2} }
\def\cWuh{ \cWvv{\bau}{3} }
\def\cWzot{ \cWvv{\baz}{12} }

\def\nWvv#1#2{ \nvprvv{#1}{\xcW} }
\def\nWzot{ \nWvv{\baz}{12} }

\def\cWuo{ \cWvv{\bau}{1} }
\def\cWwt{ \cWvv{\baw}{2} }

\def\cK{ \mdfv{K} }

\def\sE{ \shfv{E} }
%\def\mE{ \mdfv{E} }

\def\xotsq{ \otimes_{\sqcup} }
\def\xstsq{ \xcap_{\sqcup} }
\def\xobv#1{ \hat{#1} }
\def\xobwv#1{ \widehat{#1} }
\def\xobSg{ \xobv{\xSg} }
\def\xobbSg{ \xobv{\bSg} }
\def\xobM{ \xobv{\xM} }
\def\xobcbM{ \xobwv{\xbc\xM} }

\def\xobMz{ \xobwv{\stMz} }
\def\xobMo{ \xobwv{\stMo} }
\def\xobMt{ \xobwv{\stMt} }
\def\xobMth{ \xobwv{\stMth} }

\def\xobIXY{ \xobwv{\stIXY} }
\def\xobIXXpY{ \xobwv{\stIXXpY} }
\def\xobIXXpW{ \xobwv{\stIXXpW} }
\def\xobIXYYp{ \xobwv{\stIXYYp} }
\def\xobIXct{ \xobwv{\stIXct} }
\def\xobSoX{ \xobwv{\stSoX} }
\def\xobIYot{ \xobwv{\stIYot} }


\def\xobsq{ \xobwv{\sqcup} }


\def\xobN{ \xobv{\xN} }
\def\xobSo{ \xobv{S^1} }

\def\xobP{ \xobv{\xP} }

\def\xrdv#1#2{ \#_{#1,#2} }
\def\xrdij{ \xrdv{i}{j} }

\def\Dlv#1{ \Delta_{#1} }
\def\DlX{ \Dlv{\xX} }
\def\DlZ{ \Dlv{\xZ} }
\def\DlcW{ \Dlv{\ycW} }
\def\DlcY{ \Dlv{\ycY} }
\def\DlY{ \Dlv{\yY} }
\def\DlcYot{ \Dlv{\ycYaot} }
%\def\DlE{ \Dlv{\scE} }
\def\DlE{ \scE_{\DlY} }
\def\DlEv#1{ \scE_{#1,\DlY} }
\def\DlEo{ \DlEv{1} }
\def\DlEt{ \DlEv{2} }

\def\DlYoct{ \Dlv{\yYoct} }
\def\DlY{ \Dlv{\yY} }

\def\Dltrv#1{ \Dlv{#1}^{(3)} }
\def\DltrY{ \Dltrv{\yY} }
\def\strsDtrv#1{ \strs{\Dltrv{#1}} }
\def\strsDtrYoct{ \strs{\Dltrv{\yYoct} } }
\def\strsDY{ \strs{\DlY} }
\def\strsDtrY{ \strsDtrv{\yY} }
%\def\dstDv#1{ \brb{\strsDtrv{#1}}_{\shlf\sfSv{#1}} }
\def\dstDv#1{ \brb{\strsDtrv{#1}}_{\ysfStY} }
\def\dstDY{ \dstDv{\yY} }
%\def\dstDmv#1{ \brb{\strsDtrv{#1}}_{-\shlf\sfSv{#1}} }
\def\dstDmv#1{ \brb{\strsDtrv{#1}}_{-\ysfStY} }
\def\dstDYm{ \dstDmv{\yY} }



%\def\dDlESv#1{ \brb{\DlE}_{\sfSv{\yY,#1}} }
\def\dDlES{ \mtdfbv{\DlE}{\hlsfSYa} }
\def\dDlESm{ \mtdfbv{\DlE}{-\hlsfSYa} }

\def\dDlESo{ \mtdfbv{\DlEo}{\hlsfSYao} }
\def\dDlESmt{ \mtdfbv{\DlEt}{-\hlsfSYat} }

\def\xiov#1#2{ \iota_{#1,#2} }
\def\xioij{ \xiov{i}{j} }

\def\xiosv#1{ \iota_{#1} }
\def\xiosot{ \xiosv{12} }
\def\xiosth{ \xiosv{23} }
\def\xiosoh{ \xiosv{13} }

%\def\Mps{ \mathrm{Maps} }
\def\Mps{ \mathfrak{M}}
%\def\Mpsvv#1#2{ \Mps(#1\rightarrow #2) }
\def\Mpsvv#1#2{ #1\rightarrow #2 }
\def\MpsMX{ \Mpsvv{M}{\xX} }

\def\xspt{space-time}
\def\xwsh{world-sheet}
\def\xtsp{target-space}

\def\xWb{ \wedge^\bullet }
\def\rmT{ \mathrm{T} }
\def\TxX{ \rmT\xX }
\def\rmH{ \mathrm{H} }
\def\HDl{ \rmH_{\bar{\del} } }
%\def\xev{ \mathrm{even} }
\def\xev{ \bar{0} }
%\def\xod{ \mathrm{odd} }
\def\xod{ \bar{1} }
\def\xzth#1{ \hat{#1} }
\def\yev{ \xzth{0} }
\def\yod{ \xzth{1} }
\def\ypn{ \xzth{n} }
\def\zpn{ n }
\def\HDlev{ \HDl^{\yev} }
\def\HDlod{ \HDl^{\yod} }
\def\HDlevA{ \HDlev(\xcA) }

\def\dlb{ \bar{\del} }
\def\dlbp{ \dlb\p }
\def\dlbv#1{ \dlb_{#1} }
\def\dlbX{ \dlbv{\xX} }


\def\xdgav#1{ \big( \xdlAbv{#1},\dlbv{#1}\big) }
\def\xdgaX{ \xdgav{\xX} }
\def\xdgaXp{ \xdgav{\xXp} }
\def\xdgA{ (\xdlAb,\dlb) }

%\def\ydgav#1{ \big( #1, \nbbv{#1} \big) }
\def\ydgav#1{ \big( #1, \nbb \big) }
\def\ydgaA{ \ydgav{\xdlA} }

\def\ycdgav#1{ \big( #1, \nbb, \xcW \big) }
\def\ycdgaBv#1{ \Big( #1, \dlb, \xcW \Big) }
\def\ycdgaBU{ \ycdgaBv{\xbOmbU} }
\def\ycdgaBUWz{ \Big(\xbOmbU,\dlb,\xcWz \Big) }
\def\ycdgaBev#1{ \Big( #1, \dlbe, \xcWe \Big) }
\def\ycdgaBUe{ \ycdgaBev{\xbOmbU} }
\def\ycdgaA{ \ycdgav{\xdlA} }
\def\ycdgaAv#1{ \big(\xdlA,\nbb,\xcW_{#1} \big) }
\def\ycdgaAo{ \ycdgaAv{1} }
\def\ycdgaAt{ \ycdgaAv{2} }
\def\ycdgaAot{ \big(\xdlA,\nbb,\xcWo+\xcWt \big) }
\def\ycdgaAd{ \big(\xdlA,\nbb,-\xcW\big) }

\def\ycdgaBUv#1{ \Big(\xbOmbU,\dlb,#1 \Big) }
\def\ycdgaBUl{ \ycdgaBUv{\xdfm} }

\def\otdlA{ \otimes_{\xdlA} }
\def\otCbx{ \otimes_{\ICbx} }
\def\otCby{ \otimes_{\ICby} }
\def\otCbxz{ \otimes_{\ICv{\bax,\baz}} }

\def\nbbA{ \nbbv{\xdlA} }

\def\maug{\mathrm{aug}}
\def\maugv#1{ #1^{\maug} }


\def\cxM{ \mathcal{M} }
\def\cxN{ \mathcal{N} }
\def\cxP{ \mathcal{P} }
\def\xchk#1{ \check{#1} }
\def\chxP{ \xchk{\cxP} }
\def\chmP{ \xchk{\xmP} }



%\def\xcMF{ \mathrm{MF} }
%\def\xcMFd{\xcMF\!\!\!\!\!\!\!\!\!\xcMF}
\def\xcMF{ \mathsf{MF} }
\def\xcMFd{ \ddot{\xcMF} }
\def\xcMFdd{ \dddot{\xcMF} }
\def\xcMFv#1{ \xcMF_{#1} }
\def\xcMFW{ \xcMFv{\xcW} }
%\def\xcMFnz{ \xcMFv{\varnothing;0} }
\def\xcMFnz{ \xcMFvv{\varnothing}{0} }
%\def\xcMFyot{ \xcMFv{y_1,y_2;y_1^2 + y_2^2} }
\def\xcMFyot{ \xcMFvv{y_1,y_2}{y_1^2+y_2^2} }


\def\xcMFa{ \maugv{\mathsf{MF}} }
\def\xcMFad{ \maugv{\ddot{\xcMF}} }
\def\xcMFadd{ \maugv{\dddot{\xcMF}} }
\def\xcMFav#1{ \xcMFa_{#1} }
\def\xcMFaW{ \xcMFav{\xcW} }


%\def\xcMFvv#1#2{ \xcMF_{#1;#2} }
\def\xcMFvv#1#2{ \xcMF(#1;#2) }
\def\xcMFbxW{ \xcMFvv{\bax}{\xcW} }
\def\xcMFbxpW{ \xcMFvv{\baxp}{\xcW} }
\def\xcMFbxWo{ \xcMFvv{\bax}{\xcWo} }
\def\xcMFbxWt{ \xcMFvv{\bax}{\xcWt} }

\def\xcMFavv#1#2{ \xcMFa_{#1;#2} }
%\def\xcMFavv#1#2{ \xcMFa(#1;#2) }
\def\xcMFabxW{ \xcMFavv{\bax}{\xcW} }
\def\xcMFabxWo{ \xcMFavv{\bax}{\xcWo} }
\def\xcMFabxWt{ \xcMFavv{\bax}{\xcWt} }



\def\xcMFc{ \xcMF^{\smc} }
\def\xcMFcv#1{ \xcMFc_{#1} }

\def\xcMFdv#1{ \xcMFd(#1) }
\def\xcMFdbx{ \xcMFdv{\bax} }
\def\xcMFdbxp{ \xcMFdv{\baxp} }
\def\xcMFdby{ \xcMFdv{\bay} }
\def\xcMFdbz{ \xcMFdv{\baz} }
\def\xcMFdbxy{ \xcMFdv{\bax,\bay} }
\def\xcMFdbxz{ \xcMFdv{\bax,\baz} }
\def\xcMFdbyz{ \xcMFdv{\bay,\baz} }
\def\xcMFdbxxp{ \xcMFdv{\bax,\baxp} }
\def\xcMFdn{ \xcMFdv{\varnothing} }


\def\xcMFadv#1{ \xcMFad(#1) }
\def\xcMFadbx{ \xcMFadv{\bax} }
\def\xcMFadby{ \xcMFadv{\bay} }
\def\xcMFadbz{ \xcMFadv{\baz} }
\def\xcMFadbxy{ \xcMFadv{\bax,\bay} }
\def\xcMFadbxz{ \xcMFadv{\bax,\baz} }
\def\xcMFadbyz{ \xcMFadv{\bay,\baz} }

\def\xcMFbxyWs{ \xcMFvv{\bax,\bay}{\xcW(\bax) + \bay^2} }
\def\xcMFbxyWt{ \xcMFvv{\bax,\ayo,\ayt}{\xcW(\bax) + \ayo^2 +
\ayt^2} }
\def\xcMFbxpyWt{ \xcMFvv{\baxp,\ayo,\ayt}{\xcW(\baxp) + \ayo^2 +
\ayt^2} }

\def\ayots{ \ayo^2 + \ayt^2 }

\def\xcMFbvv#1#2#3{ \xcMF_{#1;#2|#3} }
\def\xcMFbxWk{ \xcMFbvv{\bax}{\xcW}{\ak} }

\def\cMF{ \mathrm{D} }
\def\cMFv#1{ \cMF_{#1} }
\def\cMFvv#1#2{ \cMFv{#1}(#2) }
\def\cMFW{ \cMFv{\xcW} }
\def\cMFAv#1{ \cMFvv{#1}{\xcA} }
\def\cMFWA{ \cMFAv{\xcW} }
\def\cMFmWA{ \cMFvv{-\xcW}{\xcA} }

%***********

%\def\xcMF{ \mathrm{MF} }
%\def\xcMFd{\xcMF\!\!\!\!\!\!\!\!\!\xcMF}
\def\xcMFA{ \mathsf{MFA} }
\def\xcMFAd{ \ddot{\xcMFA} }
\def\xcMFAdd{ \dddot{\xcMFA} }
\def\xcMFAv#1{ \xcMFA_{#1} }
\def\xcMFAW{ \xcMFAv{\xcW} }

\def\xcMFAa{ \maugv{\mathsf{MFA}} }
\def\xcMFAad{ \maugv{\ddot{\xcMFA}} }
\def\xcMFAadd{ \maugv{\dddot{\xcMFA}} }
\def\xcMFAav#1{ \xcMFAa_{#1} }
\def\xcMFAaW{ \xcMFAav{\xcW} }

%\def\xcMFAvv#1#2{ \xcMFA_{#1;#2} }
\def\xcMFAvv#1#2{ \xcMFA(#1;#2) }
\def\xcMFAbxW{ \xcMFAvv{\bax}{\xcW} }
\def\xcMFAbxpW{ \xcMFAvv{\baxp}{\xcW} }
\def\xcMFAbxWo{ \xcMFAvv{\bax}{\xcWo} }
\def\xcMFAbxWt{ \xcMFAvv{\bax}{\xcWt} }

\def\xcMFAadv#1{ \xcMFAad(#1) }
\def\xcMFAadbx{ \xcMFAadv{\bax} }

\def\xcMFAdv#1{ \xcMFAd(#1) }
\def\xcMFAdbx{ \xcMFAdv{\bax} }


%**********



\def\smc{ \mathrm{c} }
\def\cMFc{ \cMF^{\smc} }
\def\cMFcv#1{ \cMF_{#1}^{\smc} }
\def\cMFcvv#1#2{ \cMFcv{#1}(#2) }
\def\cMFcWA{ \cMFcvv{\xcW}{\xcA} }


\def\shC{ C }

%\def\xomp{ \omega_{\xp} }
\def\xO{ O }
\def\xOv#1{ \xO_{#1} }
\def\xOp{ \xOv{\xp} }

\def\xl{ l }
\def\xlin{ \xl_{\mathrm{in}} }
\def\xlout{ \xl_{\mathrm{out}} }
\def\Extb{ \Ext^\bullet }

\def\xc{ c }
\def\xcin{ \xc_{\mathrm{in}} }
\def\xcout{ \xc_{\mathrm{out}} }

\def\hdM{ \widehat{\del\xM} }
\def\hM{ \hat{\xM} }

\def\hxSg{ h_{\xSg} }



\def\drD{\xrD\!\!\!\xrD}
%\def\drDv#1{ \drD(#1) }
%
\def\xrL{ \mathrm{L} }
\def\drL{\xrL\!\!\!\xrL}
\def\drDv#1{ \drL(#1) }
%
\def\drDX{ \drDv{\xX} }
\def\drDXp{ \drDv{\xXp} }
\def\drDbv#1{ \drL\big(#1\big) }

\def\xTsv#1{ \mathrm{T}^\ast #1 }
\def\TsA{ \xTsv{\xcA} }
\def\drDTA{ \drDv{\TsA} }

\def\drDfv#1{ \drL(#1) }
\def\drDfX{ \drDfv{\xX} }
\def\drDfsA{ \drDfv{\TsA} }

\def\drDfbx{ \drDfv{\bax} }
\def\drDfby{ \drDfv{\bay} }
\def\drDfbz{ \drDfv{\baz} }
\def\drDfbxy{ \drDfv{\bax,\bay} }
\def\drDfbyz{ \drDfv{\bay,\baz} }
\def\drDfbxz{ \drDfv{\bax,\baz} }

\def\cg{ \mathrm{g} }
\def\drLg{ \drL_{\cg} }
\def\drLl{ \drL_{\mathrm{l}} }

\def\drDgv#1{ \drLg(#1) }
\def\drDgX{ \drDgv{\xX} }
\def\drDlv#1{ \drLl(#1) }
\def\drDlX{ \drDlv{\xX} }
\def\drDlTsA{ \drDlv{\TsA} }

\def\trDD{\xrD\!\!\!\xrD\!\!\!\xrD}
\def\trD{\xrL\!\!\!\xrL\!\!\!\xrL}
\def\trDg{ \trD_{\cg} }
\def\xalgg{ \mathrm{alg} }
\def\trDa{ \trD_{\xalgg} }

\def\ycY{ \mathcal{Y} }
\def\ycYv#1#2{ \ycY_{#2,#1} }
\def\ycYov#1{ \ycY_{#1} }
\def\ycYoov#1{ \yY_{#1} }
\def\ycYpv#1{ \ycYv{+}{#1} }
\def\ycYnv#1{ \ycYv{-}{#1} }
\def\ycYpi{ \ycYpv{i} }
\def\ycYni{ \ycYnv{i} }
\def\ycYpj{ \ycYpv{j} }
\def\ycYnj{ \ycYnv{j} }
\def\yZ{ Z }
\def\yY{ Y }

\def\ycYp{ \ycY\p }
\def\yYp{ \yY\p }

\def\ytcY{ \tilde{\ycY} }

\def\ycYav#1{ \ycY_{#1} }
\def\ycYo{ \ycYav{1} }
\def\ycYt{ \ycYav{2} }
\def\ycYh{ \ycYav{3} }
\def\ycYi{ \ycYav{i} }
\def\ycYj{ \ycYav{j} }

\def\yYv#1{ \yY_{#1} }
\def\yYo{ \yYv{1} }
\def\yYt{ \yYv{2} }
\def\yYh{ \yYv{3} }
\def\yYi{ \yYv{i} }
\def\yYj{ \yYv{j} }
\def\yYot{ \yYv{12} }
\def\yYij{ \yYv{ij} }
\def\yYotp{ \yYot\p }

\def\yYoct{ \yYo\cap\yYt }
\def\yYocct{ \yYo\cap\yYt }
\def\yYtch{ \yYt\cap\yYh }

\def\ycYav#1{ \ycY_{#1} }
\def\ycYao{ \ycYav{1} }
\def\ycYat{ \ycYav{2} }
\def\ycYaot{ \ycYav{12} }
\def\ycYath{ \ycYav{23} }
\def\ycYahf{ \ycYav{34} }
\def\ycYato{ \ycYav{21} }
\def\ycYatos{ \xdlv{\ycYato} }
\def\wycYaot{ \widetilde{\ycYaot} }
\def\swycYaot{ \xdlv{\wycYaot} }
\def\ycYaotp{ \ycYaot\p }
\def\ycYaotpp{ \ycYaot\pp }
\def\sycYaotp{ \xdlv{\big(\ycYaotp\big)} }

\def\xfbr#1#2#3{ \xymatrix@C=1.5pc@R=1.5pc{#1\ar[r] & #2 \ar[d] \\ & #3} }
\def\xfbrv#1#2#3#4{ \xymatrix@C=1.5pc@R=1.5pc{#1\ar[r] & #2 \ar[d]^{#4} \\ & #3} }

\def\som{ \omega }
\def\somv#1{ \som_{#1} }
\def\somo{ \somv{1} }
\def\somt{ \somv{2} }
\def\somh{ \somv{3} }
\def\Xsom{ (\xX,\som) }
\def\Xsomm{ (\xX,-\som) }
\def\Xsomv#1{ (\xXv{#1},\somv{#1}) }
\def\Xsomo{ \Xsomv{1} }
\def\Xsomt{ \Xsomv{2} }
\def\Xsomh{ \Xsomv{3} }
\def\Xsomf{ \Xsomv{4} }


%\def\xcap{ \overset{\times}{\cap} }
\def\xcap{ \boxtimes }
\def\ycapv#1{ \times_{#1} }
\def\ycapX{ \ycapv{\xX} }
\def\ycapXott{ \ycapv{(\xXott)} }
\def\ycapXsott{ \ycapv{(\xXsott)} }
\def\ycapU{ \ycapv{\xcA} }
\def\ycapUoat{ \ycapv{(\xcAo\times\xcAt)} }

\def\ycYoct{ \ycYo \ycapX \ycYt }

\def\zcap{ \boxtimes }
\def\zcap{ \tilde{\times} }
\def\zcapv#1{ \zcap_{#1} }
\def\zcapUoat{ \zcapv{(\xcAo\times\xcAt)} }
\def\zcapUaoth{ \zcapv{(\xcAo\times\xcAt\times\xcAh)} }
\def\zcapU{ \zcapv{\xcA} }
\def\zcapX{ \zcapv{\xX} }




%\def\xMor{\mathop{ \mathrm{Mor} }}
\def\xMor{\mathop{ \mathrm{Hom} }}
\def\xFun{\mathop{ \mathrm{Fun} }}
\def\xEnd{\mathop{ \mathrm{End} }}
\def\xEndv#1{ \xEnd(#1) }

\def\xMorDD{ \xMor\nolimits_{\drD} }
\def\xMorDDD{ \xMor\nolimits_{\trD} }

\def\yepi{ \pi }
\def\yepiu{ \yepi^\ast }
\def\yepiuv#1{ \yepiu_{#1} }
\def\yepiuo{ \yepiuv{1} }
\def\yepiut{ \yepiuv{2} }
\def\yepiuot{ \yepiuv{12} }
\def\yepiuth{ \yepiuv{23} }

\def\yepid{ \yepi_\ast }
\def\yepidv#1{ \yepi_{#1,\ast} }
\def\yepido{ \yepidv{1} }
\def\yepidt{ \yepidv{2} }
\def\yepidoh{ \yepidv{13} }

\def\yepiv#1{ \yepi_{#1} }
\def\yepio{ \yepiv{1} }
\def\yepit{ \yepiv{2} }
\def\yepiij{ \yepiv{ij} }
\def\yepiot{ \yepiv{12} }
\def\yepith{ \yepiv{23} }
\def\yepioh{ \yepiv{13} }
\def\yepihf{ \yepiv{34} }

\def\iotth{ \iota }
\def\xXemp{ \xX_{\varnothing} }

\def\xbc{ \del_{\mathrm{c} } }
\def\xbb{ \del_{\mathrm{b} } }
\def\dlst{ \xbc }

\def\aac{cut}
\def\aab{brane}
\def\acb{\aac\ boundary}
\def\acbs{\aac\ boundaries}
\def\abb{\aab\ boundary}
\def\abbs{\aab\ boundaries}

\def\cclsd{\aac-closed}

\def\sprt{separating}
\def\spprt{support}

\def\xsupp{ \mathop{\mathrm{supp}} }

\def\intngl{internal tangle}
\def\bntngl{boundary tangle}

\def\xal{ \alpha }
\def\xbet{ \beta }

\def\Zt{ \ZZ_2 }
\def\Ztgrdd{$\Zt$-graded}
\def\Ztgrdng{$\Zt$-grading}
\def\Zgrdd{$\ZZ$-graded}
\def\Zgrdng{$\ZZ$-grading}
\def\Ztdgr{$\Zt$-degree}
\def\Zdgr{$\ZZ$-degree}

\def\Zfltrn{$\ZZ$-filtration}

\def\dgZt{ \deg_{\Zt} }
\def\dgZ{ \deg_{\ZZ} }

\def\xPh{ \Phi }
%\def\xPhv#1{ \xPh_{#1} }
\def\xPhv#1{ \xPh\lrbs{#1} }
\def\xPhW{ \xPhv{\ycW} }
\def\xPhYot{ \xPhv{\ycYaot} }
\def\dPhYot{ \dPhv{\ycYaot} }
\def\xPhC{ \xPhv{C} }
\def\xPhF{ \xPhv{\cF} }
\def\xPhFC{ \xPhv{\cF,\shC} }
\def\xPhsF{ \xPhv{F} }
\def\xPhcF{ \xPhv{\ycF} }
\def\xPhcUWot{ \xPhv{\cmfcUWot} }

\def\xPhuv#1{ \xPh_{#1} }
\def\xPhuot{ \xPhuv{12} }
\def\xPhuotv#1{ \xPhuot\lrbs{#1} }
\def\xPhuotWzot{ \xPhuotv{\nWzot} }

\def\dPh{ \ddot{\Phi} }
%\def\dPhv#1{ \dPh_{#1} }
\def\dPhv#1{ \dPh\lrbs{#1} }
\def\dPhWzot{ \dPhv{\nWzot} }
\def\xPhWzot{ \xPhv{\nWzot} }
\def\xPhUWot{ \dPhv{\cmfnUWot} }

\def\dPhtab{ \dPhv{\nvprBvv{\baa,\ab}{\xcd{\baa}{(\baxp-\bax)}+\ab^2 }} }


%\def\xPhMot{ \xPhv{\xmMot} }
\def\xPhMot{ \xPhv{\cfMot} }
\def\xPhbxy{ \xPhv{ \xvprvv{\baz}{\xcWot} } }

\def\xPhot{ \xPhv{12} }
\def\xPhth{ \xPhv{23} }
\def\xPhEot{ \xPhv{\xcEot} }
%\def\xPhEot{ \xPhv{\acEote} }
\def\xPhEpot{ \xPhv{\xcEot\p} }
%\def\xPhEpot{ \xPhv{\acEotep} }
\def\xPhEth{ \xPhv{\xcEth} }
%\def\xPhEth{ \xPhv{\acEthe} }
\def\xPhEpth{ \xPhv{\xcEth\p} }
%\def\xPhEpth{ \xPhv{\acEthep} }

\def\xvprvv#1#2{ \lrbc{#1\,;#2} }
\def\xvprbvv#1#2{ \brb{#1\,;#2} }
\def\xvprBvv#1#2{ \brB{#1\,;#2} }

\def\nvprvv#1#2{ #1\,;#2 }
\def\nvprbvv#1#2{ #1\,;#2 }
\def\nvprBvv#1#2{ #1\,;#2 }

\def\Fib{ \mathrm{Fib} }
\def\Fibv#1{ \Fib(#1) }
\def\FibX{ \Fibv{\xX} }
\def\FibXp{ \Fibv{\xXp} }

\def\xf{ f }
\def\xfb{ \xf^\ast }
\def\xff{ \xf_\ast }

\def\xrarv#1{ \xrightarrow{\;\;#1\;\;} }

\def\any{ \forall }

\def\xdz{ d_0 }
\def\xdo{ d_1 }

\def\trfv#1{ [#1] }
\def\trfo{ \trfv{1} }

\def\tpcmpv#1#2{ \xymatrix{ #1_0\ar@<0.5ex>[r]^{\xdz} & \#1_1\ar@<0.5ex>[l]^{\xdo}
} }
\def\tpcmpE{ \tpcmpv{\cE} }


\def\xcl{cell}
\def\xclv#1{$#1$-\xcl}
\def\zcl{\xclv{0}}
\def\ocl{\xclv{1}}
\def\tcl{\xclv{2}}
\def\thcl{\xclv{3}}
\def\ncl{\xclv{n}}
\def\nmocl{\xclv{(n-1)}}
\def\npocl{\xclv{(n+1)}}
\def\icl{\xclv{i}}
\def\ipocl{\xclv{(i+1)}}
\def\imocl{\xclv{(i-1)}}

\def\xobj{object}
\def\xobjv#1{$#1$-\xobj}
\def\iobj{\xobjv{i}}
\def\zobj{\xobjv{0}}
\def\oobj{\xobjv{1}}
\def\tobj{\xobjv{2}}
\def\thobj{\xobjv{3}}
\def\nobj{\xobjv{n}}
\def\dobj{diagonal \xobj}

\def\yP{ P }

\def\oO{ O }
\def\oOO{ O\!\!O }
\def\oOOO{ O\!\!O\!\!O }

\def\stM{ \mathbf{M} }
\def\stMv#1{ \stM^{#1} }
\def\stMn{ \stMv{\zn} }
\def\stMpn{ \stMv{\prime\zn} }
\def\stMz{ \stMv{0} }
\def\stMo{ \stMv{1} }
\def\stMt{ \stMv{2} }
\def\stMth{ \stMv{3} }
\def\stMnmo{ \stMv{\zn-1} }
\def\stMnpo{ \stMv{\zn+1} }
\def\xobstM{ \xobwv{\stM} }
\def\xobstMv#1{ \xobstM^{#1} }
%\def\xobstMn{ \xobstMv{\zn} }
%\def\xobstMnpo{ \xobstMv{\zn+1} }



\def\xobstMn{ \xobwv{\stMn} }
\def\xobstMnpo{ \xobwv{\stMnpo} }
\def\xobstMth{ \xobwv{\stMth} }
\def\xobstMt{ \xobwv{\stMt} }

\def\stN{ \mathbf{N} }
\def\stNv#1{ \stN^{#1} }
\def\stNn{ \stNv{\zn} }
\def\stNnmo{ \stNv{\zn-1} }



\def\stMtbv#1#2{ \stMt_{(#1)}(#2) }
\def\stMtv#1#2{ \stMt_{#1}(#2) }
\def\stMtBv#1#2{ \stMt_{#1}\brb{#2} }
\def\stMto#1{ \stMtbv{1}{#1} }
\def\stMtt#1{ \stMtbv{2}{#1} }
\def\stMth#1{ \stMtbv{3}{#1} }
\def\stMtf#1{ \stMtv{\mathrm{ann}}{#1} }
\def\stMtBf#1{ \stMtBv{\mathrm{ann}}{#1} }
\def\stMtr#1{ \stMtv{\mathrm{rect}}{#1} }
\def\stMtrBBBC{ \stMtr{\obo,\obop,\obopp,\uC} }
\def\stMtrBBBCc{ \stMtr{\obo,\obop,\uC} }
\def\stMtrBBBCo{ \stMtr{\oboo,\oboo,\obot,\uCo} }
\def\stMtrBBBCt{ \stMtr{\obot,\obot,\oboo,\uCt} }
\def\stMtrBBBCco{ \stMtr{\oboo,\obot,\uCo} }
\def\stMtrBBBCct{ \stMtr{\obot,\oboo,\uCt} }

%***************************

\def\hstM{ \xobwv{\stM} }
\def\hstMv#1{ \hstM^{#1} }
\def\hstMn{ \hstMv{\zn} }
\def\hstMpn{ \hstMv{\prime\zn} }
\def\hstMz{ \hstMv{0} }
\def\hstMo{ \hstMv{1} }
\def\hstMt{ \hstMv{2} }
\def\hstMth{ \hstMv{3} }
%\def\hstMtbh{ \hstMbv{3} }

\def\hstMtbv#1#2{ \hstMt_{(#1)}(#2) }
\def\hstMtbbv#1#2{ \hstMt_{(#1)}\brb{#2} }
\def\hstMtbBv#1#2{ \hstMt_{(#1)}\brB{#2} }
\def\hstMtv#1#2{ \hstMt_{#1}(#2) }

\def\hstMto#1{ \hstMtbv{1}{#1} }
\def\hstMtt#1{ \hstMtbv{2}{#1} }
\def\hstMth#1{ \hstMtbv{3}{#1} }
\def\hstMtbh#1{ \hstMtbbv{3}{#1} }

\def\hstMtf#1{ \hstMtv{\mathrm{ann}}{#1} }
\def\hstMtr#1{ \hstMtv{\mathrm{rect}}{#1} }
\def\hstMtbr#1{ \hstMtbbv{\mathrm{rect}}{#1} }
\def\hstMtBr#1{ \hstMtbBv{\mathrm{rect}}{#1} }


\def\hstMtoC{ \hstMto{\uC} }

\def\hstMttB{ \hstMtt{\obo} }
\def\hstMttuW{ \hstMtt{\bau,\xcW} }
\def\hstMthBBBs{ \hstMth{\obo,\obop,\obopp} }
\def\hstMtrBBBCc{ \hstMtr{\obo,\obop,\uC} }
\def\hstMtrBBBCco{ \hstMtr{\oboo,\obot,\uCo} }
\def\hstMtrBBBCct{ \hstMtr{\obot,\oboo,\uCt} }

\def\hstMtfBC{ \hstMtf{\obo,\uC} }
\def\hstMtfBCo{ \hstMtf{\oboo,\uCo} }
\def\hstMtfBCt{ \hstMtf{\obot,\uCt} }


%***************************

\def\stMtoE{ \stMto{\cEb} }
\def\stMttYot{ \stMtt{\ycYaot} }
\def\stMthYYY{ \stMtt{\ycYaot,\ycYaotp,\ycYaotpp} }

\def\stMtoC{ \stMto{\uC} }
\def\stMttBot{ \stMtt{\oboot} }
\def\stMthBBB{ \stMtt{\oboot,\obootp,\obootpp} }


\def\stMttB{ \stMtt{\obo} }
\def\FstMttB{ \xPhv{ \hstMttB } }
\def\stMthBBBs{ \stMth{\obo,\obop,\obopp} }
\def\stMthBBBsc{ \stMth{\obo,\obo,\obop} }
\def\FstMthBBBs{ \xPhv{ \hstMthBBBs } }
\def\FstMtrBBBC{ \xPhv{ \xobwv{\stMtrBBBC} } }
\def\FstMtrBBBCc{ \xPhv{ \hstMtrBBBCc } }

\def\stMtfBC{ \stMtf{\obo,\uC} }
\def\stMtfBCo{ \stMtf{\oboo,\uCo} }
\def\stMtfBCt{ \stMtf{\obot,\uCt} }

\def\stI{ \mathbf{I} }
\def\stIv#1{ \stI_{#1} }
\def\stIXY{ \stIv{\xX;\ycY} }
\def\stIXYp{ \stIv{\xX;\ycY\p} }
%\def\stIXct{ \stIv{\xX,\mathrm{cut}} }
\def\stIXct{ \xacupv{\soptX} }
%\def\stIXXpY{ \stIv{\xX,\xXp;\ycY} }
\def\stIXXpY{ \stIv{\xXo,\xXt;\ycY} }
%\def\stIXXpW{ \stIv{\xX,\xXp;\ycW} }
\def\stIXXpW{ \stIv{\xXo,\xXt;\ycW} }
\def\stIXXpYot{ \stIv{\xXo,\xXt;\ycYaot} }
\def\stIXYYp{ \stIv{\xX;\ycY,\ycY\p} }

\def\stIYot{ \stIv{\ycYaot} }


\def\stS{ \mathbf{S} }
\def\stSo{ \stS^1 }
\def\stSov#1{ \stSo_{#1} }
\def\stSoX{ \stSov{\xX} }

\def\zc{ c }
\def\zO{ O }
\def\zOv#1{ \zO(#1) }
\def\zOc{ \zOv{\zc} }

\def\zin{ \mathrm{in} }
\def\zout{ \mathrm{out} }
\def\zcv#1{ \zc_{#1} }
\def\zcin{ \zcv{\zin} }
\def\zcout{ \zcv{\zout} }

\def\vrnv#1{ \varnothing^{#1} }
\def\vrnnmt{ \vrnv{\zn-2} }
\def\vrnnmo{ \vrnv{\zn-1} }
\def\vrnn{ \vrnv{\zn} }
\def\vrnz{ \vrnv{0} }
\def\vrno{ \vrnv{1} }


\def\xobvrnv#1{ \xobwv{\vrnv{#1}} }
\def\xobvrnmo{ \xobvrnv{-1} }
\def\xobvrnz{ \xobvrnv{0} }
\def\xobvrno{ \xobvrnv{1} }
\def\xobvrnn{ \xobvrnv{\zn} }
\def\xobvrnnmt{ \xobvrnv{\zn-2} }
\def\xobvrnnmo{ \xobvrnv{\zn-1} }
\def\xobvrnNmo{ \xobvrnv{\zN-1} }
\def\xobvrnNmt{ \xobvrnv{\zN-2} }

\def\xMan{ \mathrm{Man} }
\def\xManv#1{ \xMan_{#1} }
\def\xMann{ \xManv{\zn} }
\def\xManz{ \xManv{0} }
\def\xMano{ \xManv{1} }

\def\xIdv#1{ \xId_{#1} }
\def\xIdO{ \xIdv{\zO} }
\def\xIdA{ \xIdv{A} }
\def\xIdY{ \xIdv{\yY} }
\def\xIdYo{ \xIdv{\yYo} }
\def\xIdX{ \xIdv{\xX} }
\def\xIdXsom{ \xIdv{\Xsom} }
\def\xIdcW{ \xIdv{\ycW} }
\def\xIdcY{ \xIdv{\ycY} }
\def\xIdcYot{ \xIdv{\ycYaot} }
\def\xIdcE{ \xIdv{\cE} }
\def\xIdbx{ \xIdv{\xlobx} }


\def\xHH{ \mathop{\mathrm{HH}} }
\def\xHHv#1{ \xHH(#1) }
\def\xHHO{ \xHHv{\zO} }
\def\xHHbv#1{ \xHH\big(#1\big) }

\def\xHHub{ {\xHH}^{\bullet} }
\def\xHHubv#1{ \xHHub\brb{ #1 } }
\def\xHHYlY{ \xHHubv{\rDsprfYlY} }

%\def\Extb{ \Ext_\bullet }

%\def\zOnth{ \zO^{\varnothing} }
%\def\zOnthv#1{ \zO_{\varnothing;#1} }
\def\zOnth{ \xId_\varnothing }
\def\zOnthv#1{ \xId_{\varnothing;#1} }
\def\zOnthz{ \zOnthv{0} }
\def\zOntho{ \zOnthv{1} }
\def\zOntht{ \zOnthv{2} }
\def\zOnthh{ \zOnthv{3} }
\def\zOnthi{ \zOnthv{i} }
\def\zOnthimo{ \zOnthv{i-1} }
\def\zOnthn{ \zOnthv{\zn} }
\def\zOnthnmo{ \zOnthv{\zn-1} }
\def\zOnthNmt{ \zOnthv{\zNmt} }
\def\zOnthNmo{ \zOnthv{\zNmo} }
\def\zOnthN{ \zOnthv{\zN} }

\def\xopt{ 1-\mathrm{pt} }
\def\xoptv#1{ #1_{\xopt} }
\def\xXopt{ \xoptv{\xX} }
\def\yYopt{ \xoptv{\yY} }
\def\xcAopt{ \xoptv{\xcA} }
%\def\xXopt{ \xX_{1-\mathrm{pt}} }


\def\cO{ \mathscr{O} }
\def\cOv#1{ \cO_{#1} }
\def\cODlcW{ \cOv{\DlcW} }
\def\cODlcY{ \cOv{\DlcY} }
\def\cOX{ \cOv{\xX} }
\def\cOW{ \cOv{\yW} }
\def\cOY{ \cOv{\yY} }

\def\cODlv#1{ \cOv{\Dlv{#1}} }
\def\cODlYoct{ \cODlv{\yYoct} }

\def\Trf{ \mathcal{T} }
\def\Trfv#1{ \Trf_{#1} }
\def\TrfY{ \Trfv{\yY} }
\def\TrfYo{ \Trfv{\yYo} }
\def\TrfYt{ \Trfv{\yYt} }
\def\TrfYi{ \Trfv{\yYi} }
\def\TrfUopt{ \Trfv{\xcAopt} }
\def\TrfDlX{ \Trfv{\DlX} }
\def\TrfW{ \Trfv{\yW} }
\def\TrfU{ \Trfv{\xcA} }
\def\TrfCxot{ \Trfv{\ICxot} }
\def\TrfYopt{ \Trfv{\yYopt} }

\def\xopt{ \mathrm{1-pt} }
\def\xopt{ \text{1-pt} }
\def\xXopt{ \xX_{\xopt} }
\def\yYopt{ \yY_{\xopt} }
\def\ycYopt{ \ycY_{\xopt} }
\def\cEopt{ \cE_{\xopt} }
\def\cOopt{ \cO_{\xopt} }
\def\soptv#1{ (\xopt)_{#1} }
\def\soptX{ \soptv{\xX} }

\def\aOb{ \mathrm{Ob} }
\def\aObv#1{ \aOb_{#1} }
\def\aObi{ \aObv{i} }
\def\aObipo{ \aObv{i+1} }
\def\aObn{ \aObv{\zn} }

\def\xcmpav#1{ \big(#1\big)_\alpha }

\def\xxbcv#1#2{ \del_{\mathrm{#1}} #2 }
\def\xxbcinv#1{ \xxbcv{in} #1 }
\def\xxbcoutv#1{ \xxbcv{out} #1 }

\def\bcinstMn{ \xxbcinv{\stMn} }
\def\bcoutstMn{ \xxbcoutv{\stMn} }
\def\bcinstMo{ \xxbcinv{\stMo} }
\def\bcoutstMo{ \xxbcoutv{\stMo} }

\def\xtn{ \otimes }
%\def\xtnv#1{ \xtn_{#1} }
\def\xtnv#1{ \xtn }
\def\xtni{ \xtnv{i} }
\def\xtnipo{ \xtnv{i+1} }
\def\xtnn{ \xtnv{\zn} }
\def\xtnnpo{ \xtnv{\zn+1} }
\def\xtnz{ \xtnv{0} }
\def\xtno{ \xtnv{1} }
\def\xtnt{ \xtnv{2} }
\def\xtnh{ \xtnv{3} }

\def\xdlv#1{ #1^{\ast} }
\def\xdlE{ \xdlv{\xE} }
\def\xdlD{ \xdlv{\xtwD} }
\def\dlX{ \xdlv{\xX} }
\def\xdlbv#1{ \big( #1 \big)^\ast }
\def\xdlstMn{ \xdlbv{\stMn} }

\def\Cobv#1{ \mathrm{Cob}^#1 }
\def\CobN{ \Cobv{\zN} }
\def\CobNv#1{ \CobN(#1) }
\def\CobNC{ \CobNv{\cCmN} }
\def\Cobh{ \Cobv{3} }

\def\sin{_{\mathrm{in}} }
\def\zsin{_{\zin} }
\def\zsout{_{\zout} }

\def\xwdh{ \widehat{\;} }

\def\dstMv#1{ \xdlbv{\stMv{#1} } }
\def\dstMn{ \dstMv{\zn} }
\def\dstMnmo{ \dstMv{\zn-1} }

\def\xacap{ {\scriptstyle\bigcap} }
\def\xunitv#1{ \xId_{#1} }
\def\xacapv#1{ \xacap_{#1} }
\def\xacapstMn{ \xacapv{\stMn} }
\def\xacapA{ \xacapv{A} }
\def\xacapX{ \xacapv{\xX} }
\def\xobacapstMn{ \xobwv{\xacapstMn} }
\def\xunitstNn{ \xunitv{\stNn} }
\def\xobunitstNn{ \xobwv{\xunitstNn} }
\def\xunitstMn{ \xunitv{\stMn} }
\def\xobstNn{ \xobwv{\stNn} }
\def\capxobstMn{ \xacapv{\xobstMn} }


\def\xacup{ {\scriptstyle\bigcup} }
\def\xacupv#1{ \xacup_{#1} }
\def\xacupstMn{ \xacupv{\stMn} }
\def\xacupA{ \xacupv{A} }
\def\xacupX{ \xacupv{\xX} }
\def\xobacupstMn{ \xobwv{\xacupstMn} }


\def\zNmo{ \zN-1 }
\def\zNmt{ \zN-2 }

\def\xcC{ \mathcal{C} }
\def\xCbv#1{ \xcC\big(#1\big) }
\def\xCv#1{ \xcC(#1) }
\def\xCA{ \xCv{A} }
\def\xCB{ \xCv{B} }
\def\xCAsB{ \xCv{A^\ast\xtni B} }

\def\xcrv{\mathrm{crv}}
\def\xdrD{ \drD_{\stp} }
\def\cdrD{ \drD_{\xcrv} }
\def\cdrDv#1{ \cdrD(#1) }
\def\cdrDA{ \cdrDv{\xcA} }
\def\cdrDAo{ \cdrDv{\xcAo} }
\def\cdrDAt{ \cdrDv{\xcAt} }

\def\trDc{ \trDD_{\xcrv} }
\def\trDc{ \trD }

\def\zZ{ Z }
\def\vctc{ \text{Vect-$\IC$} }

\def\xXo{ \xX_1 }
\def\xXt{ \xX_2 }
\def\xXott{ \xXo\times\xXt }
\def\xXsott{ \dlX_1\times\xXt }

%\def\Ztgrvs{\Zt-\mathrm{gr}-\mathrm{Vect}}
\def\Ztgrvs{\text{$\Zt$-gr-Vect}}

\def\aahA{ \wedge^\bullet\bTs\xcA }

\def\HmB#1{ \Hom\Big( #1 \Big) }
\def\Hmb#1{ \Hom\big( #1 \big) }
\def\Hmo#1{ \Hom( #1 ) }

\def\XtB#1{ \Ext\Big( #1 \Big) }

\def\mF{ F }
\def\mFua{ \mF^\ast }
\def\mFda{ \mF_{\ast} }

\def\dF{ \ddot{\mF} }
\def\dFua{ \dF^\ast }
\def\dFda{ \dF_{\ast} }


\def\cFv#1{ \cF_{#1} }
\def\cFot{ \cFv{12} }
\def\cFth{ \cFv{23} }

\def\lvar#1#2{ #1_{1},\ldots,#1_{#2} }

\def\ax{ x }
\def\axv#1{ \ax_{#1} }
\def\axo{ \axv{1} }
\def\axop{ \axo\p }
\def\axt{ \axv{2} }

\def\ay{ y }
\def\ayv#1{ \ay_{#1} }
\def\ayo{ \ayv{1} }
\def\ayt{ \ayv{2} }
\def\ayop{ \ayo\p }

\def\az{ z }

\def\au{ u }
\def\aw{ w }
\def\av{ v }

\def\ap{ p }
\def\apv#1{ \ap_{#1} }
\def\apo{ \apv{1} }
\def\apt{ \apv{2} }

\def\aq{ q }

\def\aa{ a }
\def\aap{ \aa\p }
\def\af{ f }
\def\ag{ g }

\def\afMv#1{ \af_{\xmM,#1} }
\def\afcPv#1{ \af_{\cP,#1} }


\def\xR{ \ICbx }
\def\xR{ R }
\def\xRv#1{ \xR_{#1} }
\def\xRo{ \xRv{\xod} }
\def\xRz{ \xRv{\xev} }
\def\xRtt{ \xR^{\xtt} }

\def\ICbxv#1{ \ICbx_{#1} }
\def\ICbxo{ \ICbxv{\yev} }
\def\ICbxz{ \ICbxv{\yod} }

%\def\xlov#1{ [#1] }
\def\xlov#1{ #1 }
\def\xlobx{ \xlov{\bax} }
\def\xloby{ \xlov{\bay} }
\def\xlobxy{ \xlov{\bax,\bay} }
\def\xlobe{ \xlov{\varnothing} }

\def\bax{ \mathbf{\ax} }
\def\baxp{ \bax\p }
\def\baxpp{ \bax\pp }
\def\bay{ \mathbf{\ay} }
\def\baz{ \mathbf{\az} }
\def\bau{ \mathbf{\au} }
\def\baup{ \bau\p }
\def\baw{ \mathbf{\aw} }
\def\bawp{ \baw\p }
\def\bav{ \mathbf{\av} }
\def\bavp{ \bav\p }
\def\baf{ \mathbf{\af} }
\def\baa{ \mathbf{\aa} }
\def\baap{ \baa\p }

\def\ab{ b }
\def\bab{ \mathbf{\ab} }

\def\bap{ \mathbf{\ap} }
\def\baq{ \mathbf{\aq} }

\def\bafv#1{ \baf_{#1} }
\def\bafM{ \bafv{\xmM} }
\def\bafMp{ \bafv{\xmMp} }

\def\bafcP{ \bafv{\cP} }
\def\bafcPp{ \bafv{\cPp} }

\def\Koz{ \mathrm{K} }
\def\xKov#1{ \Koz\lrbc{#1} }
\def\xKobv#1{ \Koz\brb{#1} }
\def\xKoBv#1{ \Koz\brB{#1} }
\def\xKobp{ \xKov{\bap} }
\def\xKmfv#1#2{ \Koz(#1;#2) }
\def\xKmfbpq{ \xKmfv{\bap}{\baq} }
\def\xKmfbpd{ \xKmfv{\bap}{\ast} }
\def\xKpvv#1#2{ \mathrm{K}_{#1}(#2) }
\def\xKpWttbp{ \xKpvv{\xcWtt}{\bap} }

\def\vrp#1{ #1^{\prime} }
\def\vrpp#1{ #1^{\prime\prime} }

\def\baxp{ \vrp{\bax} }
\def\baxpp{ \vrpp{\bax} }

\def\baup{ \vrp{\bau} }
\def\baupp{ \vrpp{\bau} }

\def\bazp{ \vrp{\baz} }
\def\bazpp{ \vrpp{\baz} }

\def\bawp{ \vrp{\baw} }
\def\bawpp{ \vrpp{\baw} }

\def\ICv#1{ \IC[#1] }
\def\ICbx{ \ICv{\bax} }
\def\ICby{ \ICv{\bay} }
\def\ICbxy{ \ICv{\bax,\bay} }


\def\ICav#1{ \IC_{#1} }
\def\ICxv#1{ \ICav{\axv{#1}} }
\def\ICxo{ \ICxv{1} }
\def\ICxt{ \ICxv{2} }
\def\ICxi{ \ICxv{i} }
\def\ICx{ \ICav{\ax} }
\def\ICa{ \ICav{\aa} }
\def\ICxp{ \ICav{\ax,\ap} }
\def\ICp{ \ICav{\ap} }
\def\ICxot{ \ICav{\axo,\axt}^2 }

\def\ICxpv#1{ \ICav{\axv{#1},\apv{#1}}^2 }
\def\ICxpi{ \ICxpv{i} }
\def\ICxpo{ \ICxpv{1} }
\def\ICxpt{ \ICxpv{2} }
\def\ICxpot{ \IC^4_{\axo,\axt,\apo,\apt} }

\def\cbcC{ \bigcup_{\shC\in\IC} }

\def\mfM{ M }
\def\mfMv#1{ \mfM_{#1} }
\def\mfMF{ \mfMv{\cF} }
\def\mfMxo{ \mfMv{\axo} }
\def\mfMyo{ \mfMv{\ayo} }

\def\nU{ \mathcal{U} }
\def\nUv#1{ \nU_{#1} }
\def\nUx{ \nUv{x} }

\def\Tngx{ \Tng_x }

%\def\clb{ \omega }
\def\clb{ K }
\def\clbv#1{ \clb_{#1} }
\def\clbX{ \clbv{\xX} }
\def\clbU{ \clbv{\xcA} }

\def\mlb{ \cK }
\def\mlbv#1{ \mlb_{#1} }
\def\mlbX{ \mlbv{\xX} }
\def\mlbU{ \mlbv{\xcA} }




\def\cEbp{ \cEb\p }

\def\ef{ f }
\def\efv#1{ \ef_{#1} }
\def\efE{ \efv{\cE} }
\def\efEp{ \efv{\cEbp} }
\def\tcEb{ \tilde{\cEb} }

\def\zF{ F }
\def\zE{ E }

\def\txcVot{ \widetilde{\xcVot} }
\def\txcWot{ \widetilde{\xcWot} }

\def\crdf{curved differential}

\def\sa{ \alpha }
\def\sav#1{ \sa_{#1} }
\def\saU{ \sav{\xcA} }

\def\xbOmbEv#1{ \big( \xbOmbE \big)^{#1} }
\def\xbOmbEz{ \xbOmbEv{\xev} }
\def\xbOmbEo{ \xbOmbEv{\xod} }

\def\txtwDv#1{ \txtwD^{#1} }
\def\txtwDzo{ \txtwDv{\xev\xod} }
\def\txtwDoz{ \txtwDv{\xod\xev} }

\def\UId{ \nU_{\xId} }
\def\WId{ \xcW_{\xId} }

\def\smu{ \alpha }

\def\xbul{ {\bullet} }

\def\pItev#1{
\xy
(0,0)*@{*},(0,3)**@{-},(0,-3)**@{-},(5,0)*{#1}
\endxy
}
\def\pIteYot{ \pItev{\ycYaot} }
\def\pIteYto{ \pItev{\ycYato} }
\def\xobpIteYot{ \xobwv{\pIteYot} }

\def\pItevv#1#2#3{
\xy
(0,0)*{\bullet},(9,0)*{\circ}**@{-},(-9,0)*{\circ}**@{-},
(0,4)*{#3},(-9,4)*{#1},(9,4)*{#2}
\endxy
}
\def\pIteABot{ \pItevv{\obzo}{\obzt}{\oboot} }
\def\pIteABto{ \pItevv{\obzt}{\obzo}{\oboto} }

\def\pIvv#1#2{
\xy
(-5,0)*{\bullet};(5,0)*{\bullet}**@{-},
(-5,4)*{\obo},(5,4)*{\obop}
\endxy
}
\def\pIBBp{ \pIvv{\obo}{\obop} }

\def\pCtbvv#1#2{
\xy
(0,0)*\cir<10pt>{},(-3.50,0)*{\bullet},(3.50,0)*{\bullet},(-9,0)*{#1},
(9,0)*{#2}
\endxy
}

\def\pCtbBot{ \pCtbvv{\oboot}{\oboto} }

\def\pCtbvf#1#2#3#4{
\xy
(0,0)*\cir<10pt>{},(-3.50,0)*{\bullet},(3.50,0)*{\bullet},(-9,0)*{#1},
(9,0)*{#2},(0,7)*{#3},(0,-7)*{#4}
\endxy
}

\def\pCtbBotAot{ \pCtbvf{\oboot}{\oboto}{A_1}{A_2} }

\def\pCtbvo#1{
\xy
(0,0)*\cir<10pt>{},
(6,0)*{#1}
\endxy
}

\def\pCtbveo#1{
\xy
(0,0)*\cir<10pt>{},
(7,0)*{#1}
\endxy
}

\def\pCtbbveo#1{
\xy
(0,0)*\cir<10pt>{},
(13,0)*{#1}
\endxy
}

\def\pCtbA{ \pCtbvo{A} }
\def\pCtbx{ \pCtbveo{\xlobx} }
\def\pCtbXsom{ \pCtbveo{\Xsom} }
\def\pCtbX{ \pCtbveo{\xX} }
\def\pCtbTYS{ \pCtbbveo{\mtdfTYS} }

\def\pIoev#1{
\xy
(0,-1)*@{*},(0,3)**@{-},(4,-1)*{#1}
\endxy
}
\def\pIoeY{ \pIoev{\ycY} }
\def\xobpIoeY{ \xobwv{\pIoeY} }

\def\pIoev#1{
\xy
(0,-1)*@{*},(0,3)*{\circ}**@{-},(4,-1)*{#1}
\endxy
}

\def\pcrv#1{ \circ #1 }
\def\pcrA{ \pcrv{\obz} }
\def\pcrAo{ \pcrv{\obzo} }
\def\pcrAt{ \pcrv{\obzt} }

\def\psStv#1#2{
\xy
(0,0)*\cir<8pt>{},(-2.75,0)*@{*},(2.75,0)*@{*},(-7,0)*{#1},
(10,0)*{#2}
\endxy
}
\def\pStv#1#2{
\xy
(0,0)*\cir<8pt>{},(-2.75,0)*@{*},(2.75,0)*@{*},(-7,0)*{#1},
(7,0)*{#2}
\endxy
}
\def\pStYYs{ \pStv{\ycYaot}{\;\;\;\;\;\sycYaotp} }
\def\xobpStYYs{ \xobwv{\pStYYs} }
\def\pStYY{ \pStv{\ycYaot}{\ycYato} }
\def\xobpStYY{ \xobwv{\pStYY} }
%\def\pStYY

\def\xXos{ \xdlv{\xXo} }
\def\xXts{ \xdlv{\xXt} }

\def\pItv#1#2{
\xy
(-3,0)*@{*};(3,0)*@{*}**@{-},(-7,0)*{#1},(7,0)*{#2}
\endxy
}

\def\pItYY{ \pItv{\ycYao}{\ycYat} }
\def\xobpItYY{ \xobwv{\pItYY} }

\def\pSv#1{
\xy
(0,0)*\cir<8pt>{},
(7,0)*{#1}
\endxy
}

\def\pSX{ \pSv{\xX} }
\def\xobpSX{ \xobwv{\pSX} }

\def\pSv#1{ \bigcirc_{#1} }
\def\pSXo{ \pSv{ \xXo} }
\def\pSXt{ \pSv{\xXt} }

\def\iDel{ \iota_{\Delta} }
\def\yfv#1{ f_{#1} }
\def\yfo{ \yfv{1} }
\def\yft{ \yfv{2} }
\def\yfi{ \yfv{i} }

\def\xdlL{ \mathfrak{L} }
\def\xdlLv#1{ \xdlL_{#1} }
\def\xdlLa{ \xdlLv{\pga} }

\def\xdlA{ \mathcal{A} }
\def\xdlAuv#1{ \xdlA^{#1} }
\def\xdlAb{ \xdlAuv{\bullet} }
\def\xdlAe{ \xdlAuv{\yev} }
\def\xdlAo{ \xdlAuv{\yod} }
\def\xdlAZz{ \xdlAuv{0} }
\def\xdlAbv#1{ \xdlAb(#1) }
\def\xdlAbX{ \xdlAbv{\xX} }

\def\xdlAuvv#1#2{ \xdlA^{#1}(#2) }
\def\xdlAuXv#1{ \xdlAuvv{#1}{\xX} }
\def\xdlAbX{ \xdlAuXv{\bullet} }
\def\xdlAeX{ \xdlAuXv{\yev} }
\def\xdlAoX{ \xdlAuXv{\yod} }

\def\shx{ y }
\def\shbx{ \bay }

\def\xdlAv#1{ \xdlA_{#1} }
\def\xdlAx{ \xdlAv{\shx^2} }
\def\xdlAbx{ \xdlAv{\shbx^2} }

\def\nb{ \nabla }
\def\nbv#1{ \nb_{\!\!#1} }
\def\nbE{ \nbv{\xE} }
\def\nbEp{ \nbE\p }
\def\nbEot{ \nbv{\xEot} }
\def\nbEth{ \nbv{\xEth} }
\def\nbEoh{ \nbv{\xEoh} }

\def\nbb{ \bar{\nabla} }
\def\nbbv#1{ \nbb_{\!\!#1} }
\def\nbboth{ \nbbv{123} }
\def\nbbE{ \nbbv{\xE} }
\def\nbbEo{ \nbbv{\xEo} }
\def\nbbEt{ \nbbv{\xEt} }
\def\nbbEh{ \nbbv{\xEh} }
\def\nbbEi{ \nbbv{\xEi} }
\def\nbbEs{ \nbbv{\xEs} }
\def\xdgmvv#1#2{ \big(\xbOmbv{#1},\nbbv{#1} \big) }
\def\xdgmpv#1{ \big(\xbOmbv{#1},\nbbv{#1}\p \big) }
\def\xdgmdXv#1{ \big(\xbOmbv{#1},\dlbX \big) }
\def\xdgmv#1{ \xdgmvv{#1}{#1} } %%%%%%%%%% { \big(\xbOmbv{#1},\nbbv{#1} \big)}
\def\xdgsvv#1#2{ \big(#1,\nbbv{#2} \big) }
\def\xdgsv#1{ \big(#1,\nbbv{#1} \big) }
\def\xdgmE{ \xdgmv{\xE} }
\def\xdgmpE{ \xdgmpv{\xE} }
\def\xdgmEp{ \big(\xbOmbv{\xE},\nbbv{\xE}\p \big) }
\def\xdgmEo{ \xdgmv{\xEo } }
\def\xdgmEt{ \xdgmv{\xEt } }
\def\xdgmP{ \xdgsv{\xmP} }
\def\xdgmPp{ \xdgsv{\xmPp} }
\def\xdgmM{ \xdgsv{\xmM} }
\def\xdgmMo{ \xdgsv{\xmMo} }
\def\xdgmMt{ \xdgsv{\xmMt} }
\def\xdgmMp{ \xdgsv{\xmMp} }
\def\xdgmN{ \xdgsv{\xmN} }
\def\xdgmcM{ \xdgsv{\cxM} }
\def\xdgmKX{ \xdgmdXv{\clbX} }
%\big(\xbOmbv{\mlbX},\nbbv{#1} \big) }

\def\adgmv#1{ (#1,\nbbv{#1}) }
\def\adgmE{ \adgmv{\xE} }
\def\adgmEv#1{ \adgmE_{#1} }
\def\admgEzdfm{ \adgmEv{\zdfm} }
\def\adgmEo{ \adgmv{\xEo} }
\def\adgmEt{ \adgmv{\xEt} }
\def\adgmEp{ \adgmv{\xEp} }
\def\adgmpE{ (\xE,\nbbE\p) }

%\def\adgmev#1{ (#1,\nbbev{#1}) }
\def\adgmev#1{ (#1,\nbbv{#1}) }
\def\adgmeE{ \adgmev{\xE} }
\def\adgmeEp{ \adgmev{\xEp} }
\def\adgmeEo{ \adgmev{\xEo} }
\def\adgmeEt{ \adgmev{\xEt} }
\def\adgmeEh{ \adgmev{\xEh} }
\def\adgmeEot{ \adgmev{\xEot} }
\def\adgmeEpot{ \adgmev{\xEpot} }
\def\adgmeEpth{ \adgmev{\xEpth} }
\def\adgmeEth{ \adgmev{\xEth} }
\def\adgmeEoh{ \adgmev{\xEoh} }

\def\adgmzv#1{ (#1,\nbbzv{#1}) }
\def\adgmzE{ \adgmzv{\xE} }
\def\adgmzEo{ \adgmzv{\xEo} }
\def\adgmzEt{ \adgmzv{\xEt} }

\def\nbbP{ \nbbv{\xmP} }
\def\nbbM{ \nbbv{\xmM} }
\def\nbbMxo{ \nbbv{\xmMo} }
\def\nbbMxt{ \nbbv{\xmMt} }
\def\nbbN{ \nbbv{\xmN} }

\def\nbbMv#1{ \nbbv{\xmM^{#1}} }
\def\nbbMe{ \nbbMv{\yev} }
\def\nbbMo{ \nbbMv{\yod} }

\def\xdD{ D }
\def\xdDv#1{ \xdD_{#1} }
\def\xmdv#1{ \big( #1, \xdDv{#1} \big) }
\def\xsmdv#1{ (#1,\xdDv{#1} ) }
\def\xmdM{ \xmdv{\xmM} }
\def\xsmdM{ \xsmdv{\xmM} }
\def\xmdMa{ \xmdM^\ast }
\def\xmdMp{ \xmdv{\xmMp} }
\def\xmdMo{ \xmdv{\xmMo} }
\def\xmdMt{ \xmdv{\xmMt} }
\def\xsmdMo{ \xsmdv{\xmMo} }
\def\xsmdMt{ \xsmdv{\xmMt} }
\def\xdDM{ \xdDv{\xmM} }

\def\xmdfv#1{ \big( #1, \xdDv{#1}, \bafv{#1} \big) }
\def\xmdMf{ \xmdfv{ \xmM } }
\def\xmdMfp{ \xmdfv{\xmMp} }

\def\HomICv#1{ \Hom_{\ICv{#1}} }
\def\HomICbx{ \HomICv{\bax} }
\def\EndICv#1{ \End_{\ICv{#1}} }
\def\EndICbx{ \EndICv{\bax} }

\def\xIdv#1{ \xId_{#1} }








\def\xmP{ P }
\def\xmPp{ \xmP\p }
\def\xmM{ M }
\def\xmMv#1{ \xmM_{#1} }
\def\xmMo{ \xmMv{1} }
\def\xmMt{ \xmMv{2} }
\def\xmMp{ \xmM\p }
\def\xmN{ N }

\def\xmMv#1{ \xmM_{#1} }
\def\xmMot{ \xmMv{12} }
\def\xmMth{ \xmMv{23} }
\def\xmMoh{ \xmMv{13} }

\def\xmMuv#1{ \xmM^{#1} }

\def\xmPv#1{ \xmP_{#1} }
\def\xmPo{ \xmPv{1} }
\def\xmPt{ \xmPv{2} }

\def\xmrPv#1{ \xmP(#1) }
\def\xmrPv#1{ \cP(#1) }
\def\xmrPM{ \xmrPv{\cM} }

\def\Homv#1{ \Hom_{#1} }
\def\HomCh{ \Homv{\cCmh} }
\def\HomCbh{ \Homv{\Cobh} }

\def\Endv#1{ \End_{#1} }
\def\EndCh{ \Endv{\cCmh} }
\def\EndCbh{ \Endv{\Cobh} }

\def\xExt{ \Ext }
\def\xExtuv#1{ \xExt^{#1} }
\def\xExtub{ \xExtuv{\bullet} }
\def\xExtuz{ \xExtuv{0} }

\def\cmfv#1#2{ (#1,#2) }
\def\cmfBv#1#2{ \Big(#1,#2\Big) }
\def\cmfbv#1#2{ \brb{#1,#2} }
\def\cmfUW{ \cmfv{\xcA}{\xcW} }
\def\cmfUWv#1{ \cmfv{\xcA_{#1}}{\xcW_{#1}} }
\def\cmfUWo{ \cmfUWv{1} }
\def\cmfUWt{ \cmfUWv{2} }
\def\cmfUWh{ \cmfUWv{3} }

\def\cmfUWav#1{ \cmfv{\xcA}{\xcW_{#1}} }
\def\cmfUWao{ \cmfUWav{1} }
\def\cmfUWat{ \cmfUWav{2} }
\def\cmfUWah{ \cmfUWav{3} }

\def\cmfcUW{ \cmfv{\xcU}{\xcW} }
\def\cmfUW{ \cmfv{\xcA}{\xcW} }
\def\cmfUWv#1{ \cmfv{\xcAv{#1}}{\xcWv{#1}} }
\def\cmfUWo{ \cmfUWv{1} }
\def\cmfUWt{ \cmfUWv{2} }
\def\cmfcUWv#1{ \cmfv{\xcUv{#1}}{\xcWv{#1}} }
\def\cmfcUWo{ \cmfcUWv{1} }
\def\cmfcUWt{ \cmfcUWv{2} }
\def\cmfcUWh{ \cmfcUWv{3} }
\def\cmfcUWot{ \cmfcUWv{12} }
\def\cmfcUWth{ \cmfcUWv{23} }
\def\cmfcUWhf{ \cmfcUWv{34} }
\def\cmfcUWp{ \cmfv{\xcUp}{\xcWp} }

\def\cmfcUWe{ \cmfv{\xcA}{\xcWe} }
\def\cmfcUWoe{ \cmfv{\xcA}{\xcWoe} }
\def\cmfcUWte{ \cmfv{\xcA}{\xcWte} }
\def\cmfcUWhe{ \cmfv{\xcA}{\xcWhe} }
\def\cmfcYz{ \cmfv{\yY}{0} }

%\def\dmfv#1{ (#1) }
\def\dmfv#1{ #1 }
\def\dmfcUWe{ \dmfv{\xcWe} }
\def\dmfcUWpe{ \dmfv{\xcWpe} }
\def\dmfcUWoe{ \dmfv{\xcWoe} }
\def\dmfcUWte{ \dmfv{\xcWte} }
\def\dmfcUWhe{ \dmfv{\xcWhe} }
\def\dmfcUWew{ \dmfv{\xcW} }
\def\dmfcUWewo{ \dmfv{\xcWo} }
\def\dmfcUWewt{ \dmfv{\xcWt} }
\def\dmfcUWee{ \dmfv{\xcWe} }

\def\cmfcUWe{ \cmfv{\TrfU}{\xcWe} }
\def\cmfcUWew{ \cmfv{\TrfU}{\xcW} }

\def\cmfcUz{ \cmfv{\xcA}{0} }
\def\cmfcUz{ \cmfv{\TrfU}{0} }

\def\cmfcUmWv#1{ \cmfv{\xcUv{#1}}{-\xcWv{#1}} }
\def\cmfcUmWt{ \cmfcUmWv{2} }

\def\cmfcUWbsv#1{ \cmfBv{\xcUv{#1}}{p_{#1}^\ast(\xcWbsv{#1})} }
\def\cmfcUWbso{ \cmfcUWbsv{1} }
\def\cmfcUWbst{ \cmfcUWbsv{2} }

\def\cmfcUWbbsv#1{ \cmfbv{\xcUv{#1}}{p_{#1}^\ast(\xcWbsv{#1})} }
\def\cmfcUWbbso{ \cmfcUWbbsv{1} }
\def\cmfcUWbbst{ \cmfcUWbbsv{2} }

\def\nmfv#1#2{ #1,#2 }
\def\nmfBv#1#2{ #1,#2 }
\def\nmfbv#1#2{ #1,#2 }

\def\nmfUW{ \nmfv{\xcA}{\xcW} }
\def\nmfUWv#1{ \nmfv{\xcAv{#1}}{\xcWv{#1}} }
\def\nmfUWo{ \nmfUWv{1} }
\def\nmfUWt{ \nmfUWv{2} }
\def\cmfnUWv#1{ \nmfv{\xcUv{#1}}{\xcWv{#1}} }
\def\cmfnUWo{ \cmfnUWv{1} }
\def\cmfnUWt{ \cmfcUWn{2} }
\def\cmfnUWh{ \cmfcUWn{3} }
\def\cmfnUWot{ \cmfnUWv{12} }
\def\cmfnUWth{ \cmfnUWv{23} }
\def\cmfnUWhf{ \nmfcUWv{34} }
\def\cmfnUWp{ \nmfv{\xcUp}{\xcWp} }



\def\rmO{ \mathrm{O} }
\def\OnC{ \rmO(n,\IC) }
\def\OnCv#1{ \rmO(\xnv{#1},\IC) }
\def\OnYC{ \OnCv{\ycY} }

\def\xnv#1{ n_{#1} }
\def\xnY{ \xnv{\ycY} }
\def\xnYv#1{ \xnv{\ycYov{#1}} }


\def\ycF{ \cF }
\def\ycE{ \cE }
\def\ycEp{ \ycE\p }
\def\ycL{ \mathcal{L} }

\def\ycEv#1{ \ycE_{#1} }
\def\ycEo{ \ycEv{1} }
\def\ycEt{ \ycEv{2} }

\def\ycFv#1{ \ycF_{#1} }
\def\ycFot{ \ycFv{12} }
\def\ycFth{ \ycFv{23} }

\def\ak{ k }
\def\ay{ y }

\def\Exttv#1{ \Ext^{#1} }
\def\Exttev{ \Exttv{\yev} }
\def\Exttod{ \Exttv{\yod} }

\def\Extub{ \Ext^\bullet }

\def\imu{ \sqrt{-1} }

\def\xcWq{ \xcW_{\mathrm{q}} }
%\def\tcWq{ \tilde{\xcW}_{\mathrm{q}} }
\def\tcWq{ \xcW_{\mathrm{b} } }
\def\ttcWq{ \tilde{\xcW}_{\mathrm{b}} }

\def\vcL{ L }
\def\vctL{ \tilde{\vcL} }
\def\vcLs{ \vcL^{\udl} }
\def\vcLv#1{ \vcL_{#1} }
\def\vcLo{ \vcLv{1} }
\def\vcLz{ \vcLv{0} }
\def\vcLt{ \vcLv{2} }
\def\vcLot{ \vcLv{12} }
\def\vcLi{ \vcLv{i} }
\def\vcLx{ \vcLv{x} }

\def\vccL{ Q }
\def\vccLv#1{ \vccL_{#1} }
\def\vccLi{ \vccLv{i} }
\def\vccLo{ \vccLv{1} }
\def\vccLt{ \vccLv{2} }

\def\vccLd{ \dulv{\vccL} }
\def\vccLdv#1{ \vccLd_{#1} }
\def\vccLdi{ \vccLdv{i} }
\def\vccLdo{ \vccLdv{1} }
\def\vccLdt{ \vccLdv{2} }


\def\xfv#1{ f_{\mathrm{b},#1} }
\def\fvL{ \xfv{\vcL} }
\def\xafv#1{ f_{#1} }
\def\fvcE{ \xafv{\ycE} }
\def\fvcEp{ \xafv{\ycEp} }

\def\yobv#1{ \brb{#1,\xafv{#1}} }
\def\yobcE{ \yobv{\ycE} }
\def\yobcEp{ \yobv{\ycEp} }

\def\brB#1{ \Big( #1 \Big) }
\def\brb#1{ \big( #1 \big) }
\def\bro#1{ (#1) }

\def\shlf{ \tfrac{1}{2} }

\def\udl{ \ast }

\def\sfS{ S }
%\def\xsfS{ \hdf }
\def\xsfS{ \beta }
\def\xcfS{ \cdlv{\xsfS} }
\def\xsfSe{ \dfev{\xsfS} }
\def\xsfSv#1{ \xsfS_{#1} }
\def\xsfSn{ \xsfSv{\mn} }
\def\xsfSi{ \xsfSv{i} }
\def\xsfSt{ \xsfSv{2} }
\def\xsfSY{ \xsfSv{\yY} }
\def\xsfStY{ \xsfSv{2,\yY} }
\def\ysfStY{ \xsfSv{2} }
\def\ysfSY{ \xsfS }

\def\xcsfS{ \hcdf }

%\def\sfSv#1{ \sfS(#1) }
\def\sfSv#1{ \sfS_{#1} }
\def\sfSY{ \sfSv{\yY} }
\def\sfSYE{ \sfSv{\yY,\xE} }
\def\sfSYFE{ \sfSY(\acFE) }
\def\sfSYo{ \sfSv{\yYo} }
\def\sfSYt{ \sfSv{\yYt} }
\def\sfSYh{ \sfSv{\yYh} }
\def\sfSYi{ \sfSv{\yYi} }

\def\sfSvv#1#2{ \sfS(#1,#2) }

\def\sfSsv#1{ \sfS(#1) }

\def\sgrv#1#2{ \mathrm{gr}(#1,#2) }
\def\sgrMf{ \sgrv{M}{f} }

%\def\iopsTsU{ \iota\brb{p^\ast(\TsU)} }
\def\iopsTsU{ \iota\circ p^\ast(\TsU) }

%\def\xcUW{ \xcUv{\xcW} }
\def\xcUW{ \sgrv{\xcU}{\xcW} }
\def\ppt{ \tilde{p} }

\def\ypv#1{ p_{#1} }
\def\ypY{ \ypv{\ycY} }
\def\ypYi{ \ypv{\ycYi} }

\def\fpr{f}
\def\fprv#1{ \fpr|_{#1} }
\def\fprY{ \fprv{\yY} }
\def\fprYoct{ \fprv{\yYoct} }

\def\fyY{ f_{\yY} }
\def\fyYot{ f_{\yYo\cap\yYt} }

\def\DlWbs{ \Delta\xcWbs }

\def\xLC{\mathrm{LC}}
\def\xLC{\mathrm{H}^0_d}
\def\xLCv#1{ \xLC(#1) }
\def\xLCU{ \xLCv{\xcA} }
\def\xcWlc{ \xcW_{\mathrm{lc}} }

\def\vcLY{ \vcLv{\ycY} }
%\def\vcLY{ \vcLv{\yY} }
\def\vcLYv#1{ \vcLv{\ycYov{#1}} }
%\def\vcLYv#1{ \vcLv{\ycYoov{#1}} }
\def\vcLYo{ \vcLYv{1} }
\def\vcLYt{ \vcLYv{2} }
\def\vcLYh{ \vcLYv{3} }
\def\vcLYi{ \vcLYv{i} }

\def\vLY{ \vcLv{\yY} }
\def\vLYv#1{ \vcLv{\yYv{#1}} }
\def\vLYo{ \vLYv{1} }
\def\vLYt{ \vLYv{2} }


\def\govv#1#2{ \lrbc{#1,#2} }
\def\goYL{ \govv{\ycY}{\vcLY} }
\def\goYLv#1{ \govv{\ycYov{#1}}{\vcLYv{#1}} }
\def\goYLo{ \goYLv{1} }
\def\goYLt{ \goYLv{2} }
\def\goYLh{ \goYLv{3} }
\def\goYLi{ \goYLv{i} }

\def\gYL{ \govv{\yY}{\vLY} }
\def\gYLv#1{ \govv{\yYv{#1}}{\vLYv{#1}} }
\def\gYLo{ \gYLv{1} }
\def\gYLt{ \gYLv{2} }

\def\HdlbW{ \rmH_{\dlbW} }
\def\Hdlb{ \rmH_{\dlb} }
\def\HnbbE{ \rmH_{\nbbE} }
\def\Hdlbv#1{ \Hdlb^{#1} }
\def\Hdlbz{ \Hdlbv{0} }
\def\Hdlbo{ \Hdlbv{1} }
\def\Hdlbt{ \Hdlbv{2} }
\def\Hdlbb{ \Hdlbv{\bullet} }
\def\Hdlbod{ \Hdlbv{\yod} }
\def\Hdlbev{ \Hdlbv{\yev} }
\def\Hdlbi{ \Hdlbv{i} }

\def\rmS{ \mathrm{S} }
\def\StTsU{ \rmS^2\TsU }
\def\StTU{ \rmS^2\TU }
\def\TU{ \Tng\xcA }

\def\muS{ \mu_{\sfS} }

\def\mtdfv#1#2{ (#1)_{#2} }
\def\mtdfbv#1#2{ \brb{#1}_{#2} }
%\def\mtdfTUS{ \mtdfv{\TsU}{\hdf} }
\def\mtdfTUS{ \mtdfv{\TsU}{\xsfS} }
\def\mtdfTUSk{ \mtdfv{\TsU}{\hdf} }
\def\mtdfTYSk{ \mtdfv{\TsY}{\hdf} }
\def\mtdfTYoSk{ \mtdfv{\TsY_1}{\hdf} }
\def\mtdfTUh{ \mtdfv{\TsU}{\hdf} }
\def\mtdfTYS{ \mtdfv{\Ts\yY}{\ysfSY} }

\def\xEsg{ \mtdfv{\xE}{\msgm} }

\def\otOmU{ \otimes_{\xbOmbU} }
\def\otsfv#1{ \otimes_{#1} }
\def\otS{ \otsfv{\dfe\xsfS} }
\def\otS{ \otsfv{\dfe\hdf} }
\def\otSt{ \otsfv{\xsfSt} }

\def\bdmu{ \mu }
\def\bdmuv#1{ \bdmu_{#1} }
\def\bdmuot{ \bdmuv{12} }
\def\bdmuth{ \bdmuv{23} }
\def\bdmuoh{ \bdmuv{13} }
\def\bdmui{ \bdmuv{i} }
\def\bdmuo{ \bdmuv{1} }

\def\bdmuotv#1{ \bdmuv{12|#1} }
\def\bdmuotz{ \bdmuotv{0} }
\def\bdmuoto{ \bdmuotv{1} }
\def\bdmuott{ \bdmuotv{2} }

\def\tdmuotv#1{ \tilde{\bdmu}_{12|#1} }
\def\tdmuoto{ \tdmuotv{1} }
\def\tdmuott{ \tdmuotv{2} }
\def\tdmupr{ \tilde{\bdmu}_\approx }

\def\bdmua#1{ \bdmu \spsmb #1 }
\def\bdmuoha#1{ \bdmuoh \spsmb #1 }

\def\bdprv#1{ #1_{\approx} }
\def\bdmupr{ \bdprv{\bdmu} }
\def\bdnupr{ \bdprv{\bdnu} }
\def\bdxipr{ \bdprv{\bdxi} }

\def\bdnu{ \nu }
\def\bdnuv#1{ \bdnu_{#1} }
\def\bdnuot{ \bdnuv{12} }

\def\bdxi{ \xi }
\def\bdxiv#1{ \bdxi_{#1} }
\def\bdxiot{ \bdxiv{12} }



\def\bdal{ \alpha }
%\def\bdgm{ \gamma }
\def\bdgm{ \xpgv{\hdf} }

\def\Lbrv#1{ [ #1 ] }
\def\Pbrv#1{ \{ #1 \} }

\def\Hdf{Hamilton differential}
\def\hdf{\varkappa}
%\def\hdf{\beta}
\def\hdfv#1{ \hdf_{|#1} }
\def\hdfi{ \hdfv{i} }
\def\hdfj{ \hdfv{j} }
\def\hdfo{ \hdfv{1} }
\def\hdftw{ \hdfv{2} }
\def\hcdf{ \cdlv{\hdf} }
\def\hcdfv#1{ \hcdf_{|#1} }
\def\hcdfo{ \hcdfv{1} }

\def\hdfe{ \dfev{\hdf} }
\def\ehdf{ \dfe\hdf }

\def\hdfbt{ \beta }
\def\hdfgm{ \gamma }

\def\ccrR{ \check{\crR} }
\def\cdfbt{ \check{\beta} }
\def\cdfbtY{ \cdfbt_{\yY} }
\def\tdfbt{ \tilde{\beta} }
\def\tdfbtv#1{ \tdfbt_{#1} }
\def\tdfbtY{ \tdfbtv{\yY} }
\def\tdfbtYo{ \tdfbtv{\yYo} }
\def\tdfbtYt{ \tdfbtv{\yYt} }
\def\tdfbtYi{ \tdfbtv{\yYi} }
\def\tdfbtU{ \tdfbtv{\xcA} }

\def\Sta{ \mathrm{S} }
\def\Stav#1{ \Sta^{#1} }
\def\Sb{ \Stav{\bullet} }
\def\Stat{ \Stav{2} }
\def\Stah{ \Stav{3} }
\def\Stai{ \Stav{i} }
\def\Staj{ \Stav{j} }
\def\Stan{ \Stav{\mn} }
\def\StatTU{ \Stat(\TU) }
\def\SbTU{ \Sb\TU }

\def\Wb{ \wedge^{\bullet} }
\def\WbTU{ \Wb\TU }

\def\ydah{$(0,\yod)$}
\def\ydh{$(1,0)$}

\def\acR{ R }
\def\acF{ F }
\def\hacF{ \hat{F} }
\def\hacF{ \check{F} }
\def\acFv#1{ \acF_{#1} }
\def\hacFv#1{ \hacF_{#1} }
\def\hacFEo{ \hacFv{\xEo} }
\def\hacFEt{ \hacFv{\xEt} }
\def\hacFEh{ \hacFv{\xEh} }
\def\acFpv#1{ \acF\p_{#1} }
\def\acFE{ \acFv{\xE} }
\def\hacFE{ \hacFv{\xE} }
\def\acFpE{ \acFpv{\xE} }
\def\acFEp\acFv{\xEp}
\def\acFEv#1{ \acFv{\xEdv{#1}} }
\def\acFEo{ \acFv{\xEo} }
\def\acFEt{ \acFv{\xEt} }
\def\acFEh{ \acFv{\xEh} }
\def\acFEi{ \acFv{\xEi} }
\def\acFEot{ \acFv{\xEot} }
\def\acFEzot{ \acFv{\zEot} }
\def\acFEth{ \acFv{\xEth} }
\def\acFEoh{ \acFv{\xEoh} }

\def\cacF{ \check{F} }

\def\mdcd{ \mathcal{M} }
\def\mdcdv#1{ \mdcd_{#1} }
\def\mdcdE{ \mdcdv{\xE} }
\def\mdcdEo{ \mdcdv{\xEo} }
\def\mdcdEt{ \mdcdv{\xEt} }

\def\psSvv#1#2{ \left\{ #1,#2 \right\}_{\xsfSt} }
\def\psSpp{ \psSvv{\cdot}{\cdot} }

\def\dOv#1{ O_{#1} }
\def\dOk{ \dOv{k} }
\def\dOt{ \dOv{2} }
\def\dOh{ \dOv{3} }

\def\tTsU{ \widetilde{\TsU} }

\def\dfe{ \epsilon }
\def\dfev#1{ #1_{\dfe} }
%\def\dfzv#1{ #1_0 }
\def\dfzv#1{ #1 }
\def\dfzzv#1{ #1_0 }
\def\dfov#1{ #1_1 }

\def\dlbe{ \dfev{\dlb} }

\def\acEe{ \dfev{\cE} }
%\def\acEz{ \dfzv{\cE} }
%\def\acEo{ \dfov{\cE} }

\def\acEv#1{ \cE_{|\,#1} }
\def\acEz{ \acEv{0} }

\def\acEvv#1#2{ \cEv{#1\,|\,#2} }
\def\acEve#1{ \acEvv{#1}{\dfe} }
\def\acEvz#1{ \acEvv{#1}{0} }
\def\acEvo#1{ \acEvv{#1}{1} }

\def\acEoe{ \acEve{1} }
\def\acEte{ \acEve{2} }
\def\acEhe{ \acEve{3} }
\def\acEote{ \acEve{12} }
\def\acEotep{ \acEote\p }
\def\acEthe{ \acEve{23} }
\def\acEthep{ \acEthe\p }


\def\acWv#1{ \xcW_{|#1} }
\def\acWz{ \acWv{0} }
\def\acWo{ \acWv{1} }

\def\xcWe{ \dfev{\xcW} }
\def\xcWpe{ \dfev{\xcWp} }
\def\xcWz{ \dfzv{\xcW} }
\def\xcWzz{ \dfzzv{\xcW} }
\def\xcWo{ \dfov{\xcW} }

\def\xcWvv#1#2{ \xcWv{#1|#2} }
\def\xcWve#1{ \xcWvv{#1}{\dfe} }
\def\xcWvz#1{ \xcWvv{#1}{0} }
%\def\xcWvz#1{ \xcWv{#1} }
\def\xcWvo#1{ \xcWvv{#1}{1} }



\def\xcWoe{ \xcWve{1} }
\def\xcWte{ \xcWve{2} }
\def\xcWhe{ \xcWve{3} }

\def\xcWoz{ \xcWvz{1} }
\def\xcWtz{ \xcWvz{2} }
\def\xcWhz{ \xcWvz{3} }

\def\xcWote{ \xcWve{12} }
\def\xcWthe{ \xcWve{23} }
\def\xcWohe{ \xcWve{13} }

\def\xcWotz{ \xcWvz{12} }
\def\xcWthz{ \xcWvz{23} }
\def\xcWohz{ \xcWvz{13} }

\def\xcWoo{ \xcWvo{1} }
\def\xcWto{ \xcWvo{2} }
\def\xcWho{ \xcWvo{3} }
\def\xcWoto{ \xcWvo{12} }

\def\dfmvv#1#2{ #1_{#2} }

\def\dfmv#1{ \dfmvv{#1}{\bdmu} }
\def\dfmU{ \dfmv{\xcA} }
\def\xdlAm{ \dfmv{\xdlA} }
\def\nbbm{ \dfmv{\nbb} }

\def\dfmUv#1{ \dfmvv{\xcA}{#1} }
\def\dfmUmv#1{ \dfmvv{\xcA}{\bdmuv{#1}} }


\def\nbbvv#1#2{ \nbb_{#1\,|\, #2} }
\def\nbbvv#1#2{ \nbb_{#1| #2} }
\def\nbbev#1{ \nbbvv{#1}{\dfe} }
\def\nbbzv#1{ \nbbvv{#1}{0} }
%\def\nbbzv#1{ \nbb_{#1} }
\def\nbbov#1{ \nbbvv{#1}{1} }
\def\nbbeE{ \nbbev{\xE} }
\def\nbbzE{ \nbbzv{\xE} }
\def\nbboE{ \nbbov{\xE} }
\def\nbboEo{ \nbbov{\xEo} }
\def\nbboEt{ \nbbov{\xEt} }
\def\nbbeEot{ \nbbev{\xEot} }
\def\nbbeEth{ \nbbev{\xEth} }
\def\nbbeEoh{ \nbbev{\xEoh} }
\def\nbbeEo{ \nbbev{\xEo} }
\def\nbbeEt{ \nbbev{\xEt} }


\def\nbboEot{ \nbbov{\xEot} }
\def\nbboEth{ \nbbov{\xEth} }
\def\nbboEoh{ \nbbov{\xEoh} }

\def\nbbzEot{ \nbbzv{\xEot} }
\def\nbbzEth{ \nbbzv{\xEth} }
\def\nbbzEoh{ \nbbzv{\xEoh} }


\def\nbbzcxE{ \nbbzv{\cxrE} }
\def\nbbocxE{ \nbbov{\cxrE} }

\def\sea{ a }
\def\seb{ b }

\def\msgm{ \sigma }
\def\msgmv#1{ \msgm_{#1} }
\def\msgmo{ \msgmv{1} }
\def\msgmt{ \msgmv{2} }
\def\msgmbv#1{ \msgmv{|#1} }
\def\msgmbz{ \msgmbv{0} }
\def\msgmbo{ \msgmbv{1} }
\def\msgmvv#1#2{ \msgmv{#1\,|\,#2} }
\def\msgmve#1{ \msgmvv{#1}{\dfe} }
\def\msgmvz#1{ \msgmvv{#1}{0} }
%\def\msgmvz#1{ \msgmv{#1} }
\def\msgmvo#1{ \msgmvv{#1}{1} }

\def\msgmot{ \msgmv{12} }
\def\msgmote{ \msgmve{12} }
\def\msgmotz{ \msgmvz{12} }
\def\msgmoto{ \msgmvo{12} }

\def\msgmth{ \msgmv{23} }
\def\msgmthe{ \msgmve{23} }
\def\msgmthz{ \msgmvz{23} }
\def\msgmtho{ \msgmvo{23} }


\def\xIdE{ \xIdv{\xE} }

%\def\cxrv#1{ #1_{\circ} }
\def\cxrv#1{ #1 }
\def\cxrA{ \cxrv{A} }
\def\cxrmM{ \cxrv{\xmM} }
\def\cxrE{ \cxrv{\xE} }

\def\shlf{ \tfrac{1}{2} }

%\def\otS{ \otimes_{\xsfS} }

\def\TrfUZ{ (\TrfU,0) }
\def\TrfUW{ (\TrfU,\xcW) }

\def\yYW{ \yY_{\xcW} }
\def\yYWv#1{ \yY_{\xcWv{#1} }}
\def\yYWo{ \yYWv{1} }
\def\yYWt{ \yYWv{2} }
\def\yYWi{ \yYWv{i} }
%\def\yYWz{ \yYWv{0} }
\def\yYWz{ \yYWv{\dfe} }
\def\yYmu{ \yYv{\bdmu} }

\def\yYUW{ \yY_{\cmfcUW} }

\def\obz{A}
\def\obo{B}
\def\obt{C}

\def\obop{ \obo\p }
\def\obopp{ \obo\pp}

\def\obzv#1{ \obz_{#1} }
\def\obzo{ \obzv{1} }
\def\obzt{ \obzv{2} }

\def\obov#1{ \obo_{#1} }
\def\oboot{ \obov{12} }
\def\obootp{ \oboot\p }
\def\obootpp{ \oboot\pp }
\def\oboto{ \obov{21} }
\def\oboo{ \obov{1} }
\def\obot{ \obov{2} }

\def\uA{ \obz }
\def\uAv#1{ \uA_{#1} }
\def\uAo{ \uAv{1} }
\def\uAt{ \uAv{2} }
\def\uAh{ \uAv{3} }

\def\uC{ \obt }
\def\uCp{ \uC\p }
\def\uCv#1{ \uC_{#1} }
\def\uCo{ \uCv{1} }
\def\uCt{ \uCv{2} }
\def\emhat{ \hat{\;} }

\def\xcd#1#2{ #1\cdot #2 }
\def\pdq{ \xcd{\bap}{\baq} }

\def\bdel{ \boldsymbol{\del} }

\def\Cxaq{ \ICv{\bax,\baa}/(\baa-\del_{\bax}\xcW) }
\def\Cxaqo{ \ICv{\bax,\baa}/(\baa-\del_{\bax}\xcWo) }

\def\ccV{ \mathcal{V} }
\def\ccVv#1{ \ccV_{#1} }
\def\ccVann{ \ccVv{\mathrm{ann} } }
\def\ccVrc{ \ccVv{\mathrm{rect} } }

\def\xDtt{ D_{\mathrm{tot}} }

\def\rDbU{ \rDb(\xcA) }

\def\xnc#1{ \iota_{#1} }
\def\xncs#1#2{ \xnc{#1,\ast}#2 }
\def\xncY{ \xnc{\yY} }
\def\xncsY#1{ \xncs{\yY}{#1} }
\def\xncYo{ \xnc{\yYo} }
\def\xncsYo#1{ \xncs{\yYo}{#1} }
\def\xncYt{ \xnc{\yYt} }
\def\xncsYt#1{ \xncs{\yYt}{#1} }

\def\xncsDlY{ \xncs{\DlY} }
\def\xncDlY{ \xnc{\DlY} }

\def\EXsom{ \End_{\ctLLXsom} }
\def\ELYS{ \End_{\ctLLTYS} }

\def\yYph{ \yY^{\times 3} }

\def\bplijod{ \bigoplus_{i+j=\yod} }

\def\hsfSYv#1{ \widehat{\ysfStY}(#1) }
\def\hsfSYs{ \hsfSYv{\msgm} }
\def\hsfSYFot{ \hsfSYv{\acFEo-\acFEt} }
\def\hsfSYFo{ \hsfSYv{\acFEo} }
\def\hsfSYFt{ \hsfSYv{\acFEt} }
\def\hsfSYFmt{ \hsfSYv{-\acFEt} }

\def\csfSYv#1{ \widetilde{\ysfStY}(#1) }
\def\csfSYs{ \csfSYv{\msgm} }
\def\csfSYFot{ \csfSYv{\acFEo-\acFEt} }
\def\csfSYFo{ \csfSYv{\acFEo} }
\def\csfSYFt{ \csfSYv{\acFEt} }
\def\csfSYFmt{ \csfSYv{-\acFEt} }


\def\sfSYv#1{ \ysfStY(#1) }
\def\sfSYFpot{ \sfSYv{\acFEo+\acFEt} }
\def\sfSYFEzot{ \sfSYv{\acFEzot} }
\def\EotwTsY{ \zEot\otimes\wdgb\Ts\yY }
\def\EotwTY{ \zEot\otimes\wdgb\Tng\yY }
\def\wdgb{ \wedge^\bullet }

\def\zEot{ \xEot }

%\def\hlsfSY{ \shlf\sfSY }
\def\hlsfSY{ \ysfStY }
\def\hlsfSYa{ \hlsfSY(\acFE) }
\def\hlsfSYav#1{ \hlsfSY(\acFEv{#1}) }
\def\hlsfSYao{ \hlsfSYav{1} }
\def\hlsfSYat{ \hlsfSYav{2} }

\def\prT{ T }
\def\prTv#1{ T_{#1} }
\def\prTlr{ \prTv{\leftrightarrow} }
\def\prTij{ \prTv{ij} }


\def\sgpr{ \sigma }
\def\sgprv#1{ \sgpr_{#1} }
\def\sgprij{ \sgprv{ij} }

\def\St{ S_2 }
\def\Sh{ S_3 }

%\def\ttrnv#1{ \ddot{[ #1 ]} }
\def\ttrnv#1{ [#1]_2 }
\def\ttrno{ \ttrnv{1} }
\def\ttrnt{ \ttrnv{2} }
\def\ttrnn{ \ttrnv{n} }
\def\ttrnL{ \ttrnv{\vcL} }

%\def\ytrnv#1{ [ #1 ]_{\mathrm{t}} }
\def\ytrnv#1{ [ #1 ]_{\mathrm{tw}} }
\def\ytrno{ \ytrnv{1} }
\def\ytrnt{ \ytrnv{2} }
\def\ytrnn{ \ytrnv{n} }
\def\ytrnL{ \ytrnv{\vcL} }
\def\ytrnLot{ \ytrnv{\vcLot} }
\def\ytrnB{ \ytrnv{\bnB} }

\def\ztrnv#1{ \ytrnv{#1}\p }
\def\ztrno{ \ztrnv{1} }
\def\ztrnt{ \ztrnv{2} }
\def\ztrnn{ \ztrnv{n} }
\def\ztrnL{ \ztrnv{\vcL} }

%\def\ytrnso{ \ytrno{} }

\def\mV{ V }
\def\mVp{ \mV\p }
\def\mVs{ \mV^{\ast} }
\def\mSV{ \Sb\mV }
\def\mk{ k }
\def\ma{ a }
\def\mb{ b }
\def\mn{ n }
\def\mm{ m }
\def\mak{ \ma_1,\ldots,\ma_{\mk} }
\def\mbul{ \bullet }

\def\msmvv#1#2{ \lrbc{ #1 }_{#2} }
\def\msmnv#1{ \msmvv{#1}{\mn} }
\def\msmbv#1{ \msmvv{#1}{\mbul} }
\def\msmba{ \msmbv{\mak} }
\def\msmna{ \msmnv{\mak} }
\def\mp{ p }

\def\mSTUv#1{ \Stav{#1}\Tng\xcA }
\def\mSTUb{ \mSTUv{\bullet} }
\def\mSTUn{ \mSTUv{\mn} }

\def\mSTsUv#1{ \Stav{#1}\Ts\xcA }
\def\mSTsUb{ \mSTsUv{\bullet} }
\def\mSTsUn{ \mSTsUv{\mn} }
\def\mSTsUnmo{ \mSTsUv{\mn-1} }

\def\mmuv#1{ \mu_{#1} }
\def\mmuk{ \mmuv{\xsfS} }
\def\mmukn{ \mmuv{\xsfSn} }
\def\mmukt{ \mmuv{\xsfSt} }

\def\spsmb{ \,\llcorner\, }

\def\dWothzb{ (\del \xcW_{123})_{\bullet} }
%\def\nboth{ \nbbv{123} }
\def\nboth{ \zdfmv{12,23} }
\def\xtwo{ 2 }

%\def\aA{ \xdlA }
\def\aA{ \mathscr{A} }
\def\aAv#1{ \aA_{#1} }
\def\aAWvv#1#2{ \aAv{\xcWv{#1},\xcWv{#2} } }
\def\aAWot{ \aAWvv{1}{2} }
\def\aAW{ \aAv{\xcW} }
\def\aAav#1{ \aA(#1) }
\def\aAaUl{ \aAav{\xcA; \xdfm} }

\def\xmi{ i }
\def\xmj{ j }
\def\xmn{ n }
\def\xmnv#1{ \xmn_{#1} }
\def\xmno{ \xmnv{1} }
\def\xmnt{ \xmnv{2} }
\def\xmvmlt#1{$#1$-multiplication}
\def\xmnmlt{\xmvmlt{\xmn}}
\def\xmomlt{\xmvmlt{1}}
\def\xmtmlt{\xmvmlt{2}}
\def\xmvact#1{$#1$-action}
\def\xmnact{\xmvact{\xmn}}
\def\xmoact{\smvact{1}}

\def\xmm{ a }
\def\xmmbf{ \mathbf{\xmm} }
\def\xmmv#1{ \xmm_{#1} }
\def\xmmz{ \xmmv{0} }
\def\xmmo{ \xmmv{1} }
\def\xmmt{ \xmmv{2} }
\def\xmmn{ \xmmv{\xmn} }
\def\xmmnv#1{ \xmmv{\xmnv{#1}} }
\def\xmmno{ \xmmnv{1} }
\def\xmmnt{ \xmmnv{2} }

\def\ymm{ b }
\def\ymmv#1{ \ymm_{#1} }
\def\ymmz{ \ymmv{0} }
\def\ymmo{ \ymmv{1} }
\def\ymmt{ \ymmv{2} }
\def\ymmn{ \ymmv{\xmn} }

\def\zmmv#1{ \xmm^{#1} }
\def\zmmM{ \zmmv{\xmM} }
\def\zmmMv#1{ \zmmM_{#1} }
\def\zmmMz{ \zmmMv{0} }
\def\zmmMo{ \zmmMv{1} }
\def\zmmMt{ \zmmMv{2} }
\def\zmmMn{ \zmmMv{\xmn} }

\def\zmmbfv#1{ \xmmbf^{#1} }
\def\zmmbfM{ \zmmbfv{\xmM} }

\def\zmmE{ \zmmv{\xE} }
\def\zmmEv#1{ \zmmE_{#1} }
\def\zmmEz{ \zmmEv{0} }
\def\zmmEo{ \zmmEv{1} }
\def\zmmEt{ \zmmEv{2} }
\def\zmmEn{ \zmmEv{\xmn} }

\def\zmmbfE{ \zmmbfv{\xE} }




\def\zmmuMv#1{ a^{\xmMv{#1}} }
\def\zmmuMo{ \zmmuMv{1} }
\def\zmmuMt{ \zmmuMv{2} }

\def\zmf{f}
\def\zmfv#1{ \zmf_{#1} }
\def\zmfo{ \zmfv{1} }
\def\zmft{ \zmfv{2} }
\def\zmfn{ \zmfv{\xmn} }
\def\zmbf{ \mathbf{\zmf} }

\def\xmmuz{ \xmm^{(0)} }
\def\xmmbfuz{ \xmmbf^{(0)} }
\def\xmmuzv#1{ \xmmuz_{#1} }
\def\xmmuzo{ \xmmuzv{1} }
\def\xmmuzt{ \xmmuzv{2} }
\def\xmmuzn{ \xmmuzv{\xmn}}

\def\xmmuzw#1{ \xmm^{#1,(0)} }
\def\xmmuzE{ \xmmuzw{\xE} }
\def\xmmuzEv#1{ \xmmuzE_{#1} }
\def\xmmuzEo{ \xmmuzEv{1} }
\def\xmmuzEt{ \xmmuzEv{2} }
\def\xmmuzEn{ \xmmuzEv{\xmn}}

\def\xmmbfuzw#1{ \xmmbf^{#1,(0)} }
\def\xmmbfuzE{ \xmmbfuzw{\xE} }


\def\wdgb{ \wedge^\bullet }

\def\xdfm{ \lambda }
\def\xdfme{ \dfev{\xdfm} }
\def\xdfmeWW{ \xdfme(\xcWe,\xcWpe) }
%\def\xdfm{ \mu }
\def\xdfmv#1{ \xdfm_{#1} }
\def\xdfmi{ \xdfmv{i} }
\def\xdfmz{ \xdfmv{0} }
\def\xdfmo{ \xdfmv{1} }
\def\xdfmt{ \xdfmv{2} }
\def\xdfmot{ \xdfmv{12} }
\def\xdfmotij{ \xdfmv{12,ij} }
\def\xdfmY{ \xdfmv{\yY} }

\def\adfm{ \xdfm_{\cap} }
\def\adfmv#1{ \xdfm_{\cap,#1} }
\def\adfmot{ \adfmv{12} }
\def\adfmotv#1{ \adfmv{12,#1} }
\def\adfmoti{ \adfmotv{i} }
\def\adfmotz{ \adfmotv{0} }
\def\adfmoto{ \adfmotv{1} }

\def\xdfmotv#1{ \xdfmv{12,#1} }
\def\xdfmoti{ \xdfmotv{\xmi} }
\def\xdfmotn{ \xdfmotv{\xmn} }
\def\xdfmotnmo{ \xdfmotv{\xmn-1} }
\def\xdfmotz{ \xdfmotv{0} }
\def\xdfmoto{ \xdfmotv{1} }
\def\xdfmott{ \xdfmotv{2} }
\def\xdfmoth{ \xdfmotv{3} }

\def\dlbW{ \dlbv{_{\xcW}} }
\def\dlbWv#1{ \dlb #1 + \Lbrv{\xcW,#1} }

\def\hacE{ \mathrm{h}_{\acFE} }
\def\xMC{ \mathrm{MC} }
\def\MCUW{ \xMC(\xcA,\xcW) }

\def\zzal{ \alpha }
\def\zzbet{ \beta }
\def\zzV{ V }


\def\cdfm{ \cdlv{\xdfm} }
\def\cdfmv#1{ \cdfm_{#1} }
\def\cdfme{ \cdfmv{\xdfm} }
\def\cdfmo{ \cdfmv{1} }
%\def\cdfme{ \cdlv{\xdfme} }
%\def\cdfmo{ \cdlv{\xdfmo} }
\def\HdlbWUT{ \HdlbW(\xcA,\WbTU) }

\def\cEdfm{ \cE_{\cdfm} }
\def\cEdfme{ \cE_{\cdfme} }

\def\ydfm{ \mu }
\def\ydfmv#1{ \ydfm_{#1} }
%\def\ydfmo{ \ydfmv{1} }
\def\ydfmo{ \ydfm }
\def\ydfmov#1{ \ydfmo \spsmb #1 }
\def\ydfmotv#1{ \bdmuot \spsmb #1 }
\def\ycdfm{ \cdlv{\ydfm} }
\def\ycdfmv#1{ \ycdfm_{#1} }
\def\ycdfmo{ \ycdfmv{1} }

\def\zdfm{ \xcW }
\def\zdfmv#1{ \zdfm_{#1} }
\def\zdfmo{ \zdfmv{1} }
\def\zdfmz{ \zdfmv{0} }

\def\dlbm{ \dlb_{\ydfm} }

\def\dgDlb{ \deg_{\mathrm{Dlb}} }
\def\dgDlbv#1{ \dgDlb #1 }

\def\yYviv#1#2{ \yYv{#1}\cap\yYv{#2} }
\def\yYoit{ \yYviv{1}{2} }
\def\yYtih{ \yYviv{2}{3} }
\def\yYoih{ \yYviv{1}{3} }
\def\yYothi{ \yYo\cap\yYt\cap\yYh }

\def\bfp{ \mathbf{p} }

\def\Cr{ \mathrm{Cr} }
\def\Crv#1{ \Cr_{#1} }
\def\CrW{ \Crv{\xcW} }
\def\rCrW{ |_{\CrW} }
\def\CrWtmo{ \Crv{\xcWt-\xcWo} }

\def\yrl{\mathrm{rel}}
\def\dgrl{ \deg_{\yrl} }
\def\ydgm{ m }
\def\ydgn{ n }

\def\tHom{\widetilde{\Hom}}

\def\dfib{ \del_{\mathrm{vrt}} }
\def\hdft{ \tilde{\hdf} }

\def\xaV{ V }
\def\xaVs{ \xaV^\ast }
%\def\xbV{ \tilde{V} }
\def\xbV{ \xaV^\prime }
\def\xaa{ \alpha }
\def\xav{ v }
\def\xavv#1{ \xav_{#1} }
\def\xavo{ \xavv{1} }
\def\xavt{ \xavv{2} }
\def\xavh{ \xavv{3} }
\def\xaw{ w }

\def\fsd{ \del_{\mathrm{s}} }
\def\ssd{ \fsd^2 }

\def\ycfvv#1#2{ _{#1|#2} }
\def\ycfav#1{ \ycfvv{}{#1} }

\def\xcmv#1{ |_{#1} }
\def\xcmz{ \xcmv{0} }
\def\xcmo{ \xcmv{1} }
\def\xcmi{ \xcmv{i} }

\def\tcW{ \widetilde{\xcW} }
\def\tcWv#1{ \tcW_{#1} }
\def\tcWo{ \tcWv{1} }
\def\tcWt{ \tcWv{2} }
\def\hcW{ \widehat{\xcW} }
\def\hcWv#1{ \hcW_{#1} }
\def\hcWo{ \hcWv{1} }
\def\hcWt{ \hcWv{2} }
\def\tmu{ \tilde{\mu} }

\def\xcWov#1{ \xcW_{1|#1} }
\def\xcWoz{ \xcWov{0} }
\def\xcWoo{ \xcWov{1} }

\def\xcWtv#1{ \xcW_{2|#1} }
\def\xcWtz{ \xcWtv{0} }
\def\xcWto{ \xcWtv{1} }

\def\xcWotv#1{ \xcW_{12|#1} }
\def\xcWotz{ \xcWotv{0} }
\def\xcWoto{ \xcWotv{1} }

\def\hcWov#1{ \hcW_{1|#1} }
\def\hcWoz{ \hcWov{0} }
\def\hcWoo{ \hcWov{1} }

\def\hcWtv#1{ \hcW_{2|#1} }
\def\hcWtz{ \hcWtv{0} }
\def\hcWto{ \hcWtv{1} }

\def\hcWot{ \hcW_{12} }

\def\hcWotv#1{ \hcW_{12|#1} }
\def\hcWotz{ \hcWotv{0} }
\def\hcWoto{ \hcWotv{1} }

\def\bdnuotv#1{ \bdnu_{12|#1} }
\def\bdnuotz{ \bdnuotv{0} }
\def\bdnuoto{ \bdnuotv{1} }
\def\bdnuott{ \bdnuotv{2} }

\def\bdxiotv#1{ \bdxi_{12|#1} }
\def\bdxiotz{ \bdxiotv{0} }
\def\bdxioto{ \bdxiotv{1} }
\def\bdxiott{ \bdxiotv{2} }

\def\vrx{ x }
\def\vrxv#1{ \vrx^{#1} }
\def\vrxI{ \vrxv{\inI} }
\def\vrxJ{ \vrxv{\inJ} }
\def\vrxK{ \vrxv{\inK} }

\def\inI{ I }
\def\inJ{ J }
\def\inK{ K }
\def\inL{ L }
\def\inM{ M }
\def\vrxI{ \vrxv{\inI} }

\def\dlv#1{ \del_{#1} }
\def\dlI{ \dlv{\inI} }
\def\dlJ{ \dlv{\inJ} }
\def\dlK{ \dlv{\inK} }
\def\dlL{ \dlv{\inL} }
\def\dlM{ \dlv{\inM} }

\def\nbcv#1{ \nabla_{#1} }
\def\nbcI{ \nbcv{\inI} }
\def\nbcJ{ \nbcv{\inJ} }
\def\nbcK{ \nbcv{\inK} }
\def\nbcL{ \nbcv{\inL} }
\def\nbcM{ \nbcv{\inM} }

\def\crR{ R }

\def\OWv#1{ O(\xcW^{#1}) }
\def\OWz{ \OWv{0} }
%\def\OWo{ \OWv{1} }
\def\OWo{ O(\xcW) }
\def\OWt{ \OWv{2} }
\def\OWh{ \OWv{3} }
\def\OWn{ \OWv{n} }

\def\xcAekot{ \xcA_{\dfe\bdmuot} }
\def\xcAekth{ \xcA_{\dfe\bdmuth} }
\def\xcAekoh{ \xcA_{\dfe\bdmuoh} }

\def\xcEbz{ \xcE_{|0} }
\def\xcEvbz#1{ \xcE_{#1|0} }
\def\xcEobz{ \xcEvbz{1} }
\def\xcEtbz{ \xcEvbz{2} }

\def\shdfv#1{ \hdf_{#1} }
\def\shdfij{ \fsd\shdfv{ij} }
\def\shdfijk{ \ssd\shdfv{ijk} }
\def\shdfot{ \fsd\shdfv{12} }
\def\shdfoth{ \ssd\shdfv{123} }

\def\dulv#1{ #1\check }
\def\bnB{ B }
\def\bntB{ \tilde{\bnB} }
\def\bnBd{ \dulv{\bnB} }
\def\fWv#1{ \xcW_{#1} }
\def\fWbnB{ \fWv{\bnB} }

\def\tbw{ {\textstyle \bigwedge} }
\def\xtbw{ \tbw }
\def\wdtpv#1{ {\textstyle \bigwedge}^{\mathrm{ top}} #1 }
\def\wdtpB{ \wdtpv{\bnB} }
\def\Cr{ \mathop{\mathrm{Crit}} }
\def\Crv#1{ \Cr(#1) }
\def\CrWz{ \Crv{\xcWz} }
\def\CrW{ \Crv{\xcW} }
%\def\xcAWz{ \CrWz }

\def\edfn{ := }


\def\cnKv#1{ K_{#1} }
\def\cnKY{ \cnKv{\yY} }
\def\cnKU{ \cnKv{\xcA} }
\def\cnKYot{ \cnKv{\yYot} }
\def\cnKYi{ \cnKv{\yYi} }
\def\cnKYo{ \cnKv{\yYo} }
\def\cnKYt{ \cnKv{\yYt} }
\def\cnKYij{ \cnKv{\yYij} }

\def\yYoti{ \yYot }
\def\yYoct{ \yYoti }

\def\dulv#1{ #1^{\vee} }
\def\xdulv#1{ \dulv{#1} }
\def\ott{ ^{\otimes 2} }

\def\Vd{ \dulv{\xaV} }

\def\TY{ \Tng\yY }
\def\NY{ \Nrm\yY }
\def\TsY{ \Ts\yY }

\def\TsUhdf{ (\TsU)_\hdf }

\def\xfu{ u }
\def\xfVv#1{ \Vfbv{#1} }
\def\xfVu{ \xfVv{\xfu} }
\def\crcUv#1{ \xcU_{#1} }
\def\crcUW{ \crcUv{\xcW} }

\def\mpf{ f }
\def\zzf{ g }
\def\zzfv#1{ \zzf_{#1} }
\def\zzfo{ \zzfv{1} }
\def\zzft{ \zzfv{2} }
\def\zzfot{ \zzfv{12} }
\def\zzfi{ \zzfv{i} }

\def\yobYWv#1{ (\yYWv{#1},\zzfv{#1}^\ast\vcLz) }
\def\yobYWo{ \yobYWv{1} }
\def\yobYWt{ \yobYWv{2} }

\def\xcX{ \mathcal{X} }
\def\xcXv#1{ \xcX_{#1} }
\def\xcXo{ \xcXv{1} }
\def\xcXt{ \xcXv{2} }
\def\xcXh{ \xcXv{3} }
\def\xcXopt{ \xcXv{\xopt} }

\def\xs{ s }
\def\xsv#1{ \xs_{#1} }
\def\xso{ \xsv{1} }
\def\xst{ \xsv{2} }
\def\xsopt{ \xsv{\xopt} }

\def\zNc{$\zN$-category}
\def\zNcmo{$(\zN-1)$-category}
\def\zNcmos{$(\zN-1)$-categories}
\def\zdlv#1{ #1^{\hve} }

\def\HomC{ \Hom_{\cC} }

\def\cCov#1{ \cC_{#1} }
\def\cCX{ \cCov{\xcX} }
\def\cCXo{ \cCov{\xcXo} }
\def\cCXt{ \cCov{\xcXt} }

\def\Tvs{ \rmT^\vee }

\def\xfp{ p }
\def\yZv#1{ \yZ_{#1} }
\def\yZo{ \yZv{1} }
\def\yZt{ \yZv{2} }

\def\tpct{2-periodic category}
\def\HomLXom{ \Hom_{\ctLLXsom} }

\def\xzobj{object}
\def\xzobjs{\xzobj s}

\def\zdgz#1{ |#1|_{\ZZ} }
\def\zdgt#1{ |#1| }

\def\xblnk{ - }

\def\IdW{ \xIdv{\xcW} }
\def\IdbxW{ \xIdv{\bax;\xcW} }

\def\dLt{ \ddot{\Lambda} }
\def\dLtp{ \dLt_+ }
\def\dLtm{ \dLt_- }
\def\dLtpm{ \dLt_\pm }

\def\dId{ \ddot{\xId} }
\def\dIdv#1{ \dId_{#1} }
\def\Idba{ \dIdv{\baa} }

\def\ocW{ \xcW }
\def\ocWv#1{ \ocW_{#1} }
\def\ocWo{ \ocWv{1} }
\def\ocWt{ \ocWv{2} }
\def\ocWh{ \ocWv{3} }

\def\HmMFbx{ \Hom_{\xcMFdbx} }
\def\HmDDU{ \Hom_{\rDDprfU} }
\def\HmDDaU{ \Hom_{\rDDprfaU} }

\def\xFib{ \mathrm{Fib} }
\def\xFibv#1{ \xFib_{#1} }
\def\xFibx{ \xFibv{x} }
\def\FCrit{ \mathrm{FibCrit} }
\def\Sprt{ \mathop{\mathrm{Supp} } }

\def\xcWnl{ \xcW_0 }
%\def\mgv#1{ g_{#1} }
\def\mgv#1{ g }

\def\dgdW{ \deg_{\del\xcW} }
\def\spdg{ \deg_{\mathrm{sc}} }

\def\xblnk{ - }

\def\tnsct{ \tau }
\def\bnbl{ \boldsymbol{\nabla} }
\def\Tfl{ \mathcal{T} }
\def\Tflvv#1#2{ \Tfl^{#1}_{#2} }
\def\ixk{ k }
\def\ixl{ l }
\def\Tflkl{ \Tflvv{\ixk}{\ixl} }
\def\TflklU{ \Tflkl(\xcA) }
\def\Tflbb{ \Tflvv{\bullet}{\bullet} }
\def\TflbbU{ \Tflbb(\xcA) }
\def\xTfl{ \Tfl }
\def\xTflU{ \xTfl(\xcA) }
\def\Tflnb{ \Tfl_{\bnbl} }
\def\Tflnbot{ \Tfl_{\bnbl,12} }
\def\Tflnv#1{ \Tflnb[#1] }

\def\dgkp{ \deg_{\hdf} }
\def\dgbl{ \deg_{\mathrm{bal}} }
\def\dgdf{ \deg_{\mathrm{tot}} }

\def\eE{ E }
\def\eEv#1{ \eE_{#1} }
\def\eEo{ \eEv{1} }
\def\eEt{ \eEv{2} }
\def\eEh{ \eEv{3} }

\def\dfal{ \alpha }
\def\dfal{ \zeta }
\def\dfalv#1{ \dfal_{#1} }
\def\dfalot{ \dfalv{12} }
\def\dfalotv#1{ \dfalv{12,#1} }
\def\dfaloto{ \dfalotv{1} }
\def\dfalott{ \dfalotv{2} }
\def\dfaloth{ \dfalotv{3} }
\def\dfalotf{ \dfalotv{5} }
\def\dfaloti{ \dfalotv{i} }


\def\baxp{ \bax\p }
\def\bayp{ \bay\p }

\def\xcApv#1{ \xcA\p_{#1} }



\def\xcAbx{ \xcAv{\bax} }
\def\xcApbx{ \xcAp_{\bax} }
\def\xcAmbx{ \xcAv{-\bax} }
\def\xcApbxp{ \xcApv{\baxp} }
\def\xcApmbxp{ \xcApv{-\baxp} }
\def\xcApbyp{ \xcApv{\bayp} }
\def\xcApmbyp{ \xcApv{-\bayp} }
\def\ICnbv#1{ \IC^{\zn}_{#1} }
\def\ICnbax{ \ICnbv{\bax} }
\def\ICnbay{ \ICnbv{\bay} }
\def\xcVv#1{ \xcV_{#1} }
\def\xcVbx{ \xcVv{\bax} }
\def\xcVby{ \xcVv{\bay} }
\def\xcVmby{ \xcVv{-\bay} }
\def\xcVpv#1{ \xcV\p_{#1} }
\def\xcVpbxp{ \xcVpv{\baxp} }
\def\xcVpbyp{ \xcVpv{\bayp} }
\def\xcVpmbyp{ \xcVpv{-\bayp} }

\def\xcAxv#1{ \xcAv{#1,\bax_{#1}} }
\def\xcVyv#1{ \xcVv{#1,\bay_{#1}} }
\def\xcAxo{ \xcAxv{1} }
\def\xcAxt{ \xcAxv{2} }
\def\xcAxh{ \xcAxv{3} }
\def\xcVyo{ \xcVyv{1} }
\def\xcVyt{ \xcVyv{2} }
\def\xcVyh{ \xcVyv{3} }


\def\UxVyo{ \xcAxo\times\xcVyo }
\def\UxVyt{ \xcAxt\times\xcVyt }
\def\UxVyh{ \xcAxh\times\xcVyh }

\def\TsUbx{ \Ts\xcAbx }

\def\UxVy{ \xcAbx\times\xcVby }
\def\UpxVy{ \xcApbx\times\xcVby }
\def\UmxVmy{ \xcAmbx\times\xcVmby }
\def\VyUx{ \xcVby\times\xcAbx }
\def\VmyUx{ \xcVmby\times\xcAbx }
\def\VyUmx{ \xcVby\times\xcAmbx }
\def\UxVypp{ \xcApbxp\times\xcVpbyp }
\def\sUV{ \xcA\times\xcV }
\def\sUVpp{ \xcAp\times\xcVp }
\def\zsq{ q }
\def\zsp{ p }
\def\qfib{$\zsq$-fibration}
\def\pfib{$\zsp$-fibration}
\def\qemb{$\zsq$-embedding}
\def\pemb{$\zsp$-embedding}
\def\smrc{symplectic rectangle}
\def\rcch{rectangular chart}

\def\hrq{\hookrightarrow_{\zsq} }


\def\sfq{ \varepsilon }
\def\rfq{ \sfq_{\zsq} }
\def\sfqv#1{ \sfq_{#1} }
\def\sfqth{ \sfqv{23} }
\def\sfqot{ \sfqv{12} }
\def\sfqoh{ \sfqv{13} }


%\def\hve{ \vee }
%\def\hve{ \spadesuit }
\def\hve{ \diamondsuit }

\def\xtsm{ \tau }
\def\ddxtsm{ \ddot{\xtsm} }
\def\xtsmo{ \xtsm_1 }
\def\ddxtsmo{ \ddxtsm_1 }

\def\TsUv#1{ \Ts\xcAv{#1} }
\def\TsUo{ \TsUv{1} }
\def\TsUt{ \TsUv{2} }

\def\etfe{ \ddot{\mathsf{E}} }
\def\etfe{ \dPh_{\cong} }
\def\etfev#1{ \dPh_{\cong,#1} }
\def\etfeot{ \etfev{12} }
\def\etfeo{ \etfev{1} }
\def\etfet{ \etfev{2} }

\def\prms{ \sigma }

\def\rsf{ \dPh_{ \mathrm{r} } }
\def\rsfv#1{ \dPh_{ \mathrm{r},#1 } }
\def\rsfo{ \rsfv{1} }
\def\rsft{ \rsfv{2} }
\def\rsfe{ \rsfv{\sfq} }

\def\xemq{ \hookrightarrow_q }

%\def\semq{ \varepsilon }

\def\mch{ f }

\def\prsf{ \ddot{\mathfrak{P}} }
\def\prsfv#1{ \prsf #1 }
\def\prsfXsom{ \prsfv{\Xsom} }

\def\zzO{ O }
\def\zzOv#1{ \zzO_{#1} }
\def\zzOf{ \zzOv{\mch} }
\def\zzOfp{ \zzOv{\mch\p} }

\def\zzOo{ \zzOv{1} }
\def\zzOt{ \zzOv{2} }

\def\zzOfv#1{ \zzOv{#1,\mch_{#1} } }
\def\zzOfo{ \zzOfv{1} }
\def\zzOft{ \zzOfv{2} }

\def\ftnt#1{ \footnote{#1} }

\def\hsnv#1{ \del^2 #1 }
\def\hsnW{ \hsnv{\xcW} }
\def\hsnWb{ (\hsnW) }

\def\xEndsp{ \End_{\rDDprfUSk}(\zsU) }

\def\nbbEav#1{ \nbbv{\xE,#1} }
\def\nbbEai{ \nbbEav{i} }
\def\nbbEaz{ \nbbEav{0} }
\def\nbbEao{ \nbbEav{1} }
\def\nbbEat{ \nbbEav{2} }

\def\zdfm{ \zeta }
\def\zdfmv#1{ \zdfm_{#1} }
\def\zdfmo{ \zdfmv{1} }
\def\zdfmt{ \zdfmv{2} }
\def\zdfmn{ \zdfmv{\xmn} }
\def\zdfmi{ \zdfmv{i} }
\def\zdfmot{ \zdfmv{12} }
\def\zdfmoth{ \zdfmv{123} }
\def\zdfmothv#1{ \zdfmv{123,#1} }
\def\zdfmothn{ \zdfmothv{\xmn} }
\def\zdfmothp{ \zdfmoth\p }
\def\zdfmothnp{ \zdfmothn\p }

\def\tzdfm{ \tilde{\zdfm} }
\def\tzdfmv#1{ \tzdfm_{#1} }
%\def\tzdfmoth{ \tzdfmv{123} }
\def\tzdfmoth{ \tzdfmv{123,\xmn} }

\def\zdfmotv#1{ \zdfmv{12,#1} }
\def\zdfmoti{ \zdfmotv{i} }
\def\zdfmotn{ \zdfmotv{\xmn} }
\def\zdfmoto{ \zdfmotv{1} }
\def\zdfmott{ \zdfmotv{2} }

\def\zdfmdv#1{ \zdfm[#1] }
\def\zdfmdvv#1#2{ \zdfm_{#1}[#2] }
\def\zdfmdnv#1{ \zdfmdvv{\xmn}{#1} }

\def\zas{ \alpha }
\def\zasv#1{ \zas_{#1} }
\def\zasoth{ \zasv{123} }
\def\zasothv#1{ \zasv{123,#1} }
\def\zasothi{ \zasothv{i} }
\def\zasothn{ \zasothv{\xmn} }
\def\zasotht{ \zasothv{2} }

\def\ycrc{ \circ }

\def\dgF{ \deg_{\acF} }
\def\dgbt{ \deg_{\hdfbt} }

\def\xIdEm{ \xIdv{\xEo\otimes\xEt\otimes\xEh} }

\def\adlt{ \delta }
\def\adltv#1{ \adlt_{#1} }
\def\adltoth{ \adltv{123} }
\def\adltothzn{ \adltoth\zdfmn }

\def\xO{ \mathcal{O} }
\def\xOv#1{ \xO_{#1} }
\def\xOot{ \xOv{12} }

\def\xfob{fibration object}

\def\xkk{ k }

\def\zsU{ 0_{\xcA} }
\def\wsU{ \TrfUZ }

\def\btrno{ \ttrno }
\def\btrnt{ \ttrnt }
\def\btrnn{ \ttrnn }
\def\btrnv#1{ \ttrnv{#1} }

\def\ctrnv#1{ \btrnv{#1}\p }
\def\ctrno{ \ctrnv{1} }
\def\ctrnt{ \ctrnv{2} }
\def\ctrnn{ \ctrnv{n} }


==> defs/locdefgr.tex <==
\def\lcir{
\xygraph{
!{0;/r1pc/:}
[l(1.2)u(0.25)]
{\vcap-}
{\vcap}
}
}

\def\lxnv#1{\xybox{0;/r1pc/:(0,0)*{#1},(-0.7,-0.5)*{},(0.9,-0.5)*{},(0,1.1)*{},(0,-1)*{}}
}

\def\lxcir{ \lxnv{\lcir} }
%\def\hlcir{ \mfgrv{\lxcir} }
\def\hlcir{ \symalg{\lxcir} }

\def\hlcir{ \symalg{
\xybox{0;/r1pc/:
(-10.6,3.7)*{\xygraph{
!{0;/r1.5pc/:}
[l(1.5)d(0.5)]
!{\vcap-}
!{\vcap}
}
},
(-11,3)*{},
(-10.5,3)*{}
}
} }

\def\hlcir{
\xygraph{
!{0;/r1.5pc/:}
%[l(1.5)d(0.5)]
!{\vcap-}
!{\vcap}
[u(0.75)r(0.53)]
%{\cir<2pt>{}}
*{\bullet}
}
}

\def\chlcir{
\xygraph{
!{0;/r1.5pc/:}
%[l(1.5)d(0.5)]
!{\vcap-}
!{\vcap}
[u(0.75)r(0.53)]
%{\cir<2pt>{}}
*{\circ}
}
}


==> defs/locdefgr2.tex <==
\def\hlcir{
\xygraph{
!{0;/r1.5pc/:}
%[l(1.5)d(0.5)]
!{\vcap-}
!{\vcap}
[u(0.75)r(0.53)]
%{\cir<2pt>{}}
*{\bullet}
}
}

\def\chlcir{
\xygraph{
!{0;/r1.5pc/:}
%[l(1.5)d(0.5)]
!{\vcap-}
!{\vcap}
[u(0.75)r(0.53)]
%{\cir<2pt>{}}
*{\circ}
}
}

\def\lcir{
\xygraph{
!{0;/r1.5pc/:}
%[l(1.5)d(0.5)]
!{\vcap-}
!{\vcap}
%[u(0.75)r(0.53)]
%*{\bullet}
}
}

\def\xcrsp{
\xygraph{
!{0;/r1.5pc/:}
[u(0.5)]
!{\xoverv}
%[u(1.5)r(0.53)]
%*{\bullet}
}
}

\def\xpver{
\xygraph{
!{0;/r1.5pc/:}
[u(0.5)]
!{\xunoverv}
%[u(1.5)r(0.5)]
%*{\smalg}
}
}

\def\xphor{
\xygraph{
!{0;/r1.5pc/:}
[u(0.5)]
!{\xunoverh}
%[u(0.5)l(0.5)]
%*{\smalg}
}
}

\def\xvfro{
\xygraph{
!{0;/r1.5pc/:}
[u(0.5)]
!{\xcapv@(0)}
[u(1.5)]
%*{\smalg}
[u(0.45)r(0.23)]
[d(1.5)]
*{\symfr\;\scriptstyle{1}}
%[u(1.5)]
%*{\bullet}
}
}

\def\xvert{
\xygraph{
!{0;/r1.5pc/:}
[u(0.5)]
!{\xcapv@(0)}
}
}


\def\gbr{
\xygraph{
!{0;/r0.75pc/:}
!{\hcrossneg}
!{\hcrossneg}
}
}

\def\gbrv#1#2#3{
\xygraph{
!{0;/r0.75pc/:}
[u(0.5)]
!{\hcrossneg}
!{\hcrossneg}
[l(1)u(0.5)]
*{\scriptstyle{#1}}
[d(1)r(#3)]
*{\scriptstyle{#2}}
}
}



\def\gbrmv#1#2{ \gbrv{m}{#1}{#2} }
\def\gbrmn{ \gbrmv{n}{2} }
\def\gbrmnmt{ \gbrmv{n-2}{2.5} }

\def\abrmn{ \bsymalg{\;\gbrmn} }
\def\cbrmns{ \bsymcats{\;\gbrmn} }

\def\cbrmnmtps{ \bsymcatps{\;\gbrmnmt} }
\def\cbrmnmts{ \bsymcats{\;\gbrmnmt} }

\def\gbrov#1#2{ \gbrv{1}{#1}{#2} }
\def\gbron{ \gbrov{n}{2} }
\def\gbronmt{ \gbrov{n-2}{2.5} }

\def\abron{ \bsymalg{\;\gbron} }
\def\cbrons{ \bsymcats{\;\gbron} }

\def\gbrmov#1#2{ \gbrv{m+1}{#1}{#2} }
\def\gbrmon{ \gbrmov{n}{2} }
\def\gbrmonmt{ \gbrmov{n-2}{2.5} }

\def\abrmon{ \bsymalg{\;\gbrmon} }
\def\cbrmons{ \bsymcats{\;\gbrmon} }

\def\gcapv#1#2#3{
\xygraph{
!{0;/r0.75pc/:}
[u(0.5)]
!{\hcap-}
[u(0.5)]
*{\scriptstyle{#2}}
[d(1)r(#3)]
*{\scriptstyle{#1}}
}
}

\def\gcapvi#1#2{ \gcapv{#1}{i}{#2} }
\def\gcapni{ \gcapvi{n}{0.75} }

\def\acapni{ \bsymalg{\gcapni} }
\def\ccapni{ \bsymcat{\!\gcapni} }

\def\gcapvI#1#2{ \gcapv{#1}{\stI}{#2} }
\def\gcapnI{ \gcapvI{n}{0.75} }
\def\ccapnI{ \bsymcat{ \gcapnI } }

%\def\gcapnit{ \gcapv{n}{i;2}{0.75} }

\def\gcapfv#1#2#3#4{
\xygraph{
!{0;/r0.75pc/:}
[u(0.5)]
!{\hcap-}
[u(0.5)]
*{\scriptstyle{#2}}
[l(0.5)d(1)]
*{\circ}
[l(0.75)]
*{\scriptstyle{#3}}
[r(#4)]
*{\scriptstyle{#1}}
}
}

\def\gcapnit{ \gcapfv{n}{i}{2}{2} }
\def\gcapnik{ \gcapfv{n}{i}{k}{2} }

\def\gcupv#1#2#3{
\xygraph{
!{0;/r0.75pc/:}
[u(0.5)]
!{\hcap}
[u(0.5)]
*{\scriptstyle{#2}}
[d(1)r(#3)]
*{\scriptstyle{#1}}
}
}

\def\gcupvi#1#2{ \gcupv{#1}{i}{#2} }
\def\gcupni{ \gcupvi{n}{-0.75} }

\def\acupni{ \bsymalg{\gcupni} }
\def\ccupni{ \bsymcat{\gcupni\!} }

\def\gcupvI#1#2{ \gcupv{#1}{\stI}{#2} }
\def\gcupnI{ \gcupvI{n}{-0.75} }
\def\ccupnI{ \bsymcat{ \gcupnI } }

\def\gcupvIp#1#2{ \gcupv{#1}{\stI\p}{#2} }
\def\gcupnIp{ \gcupvIp{n}{-0.75} }
\def\ccupnIp{ \bsymcat{\gcupnIp} }

\def\gidbrv#1#2{
\xygraph{
!{0;/r0.75pc/:}
[u(0.8)]
!{\xcaph@(0)}
[d(1.5)l(1)]
!{\xcaph@(0)}
[u(1)l(0.4)]
*{\vdots}
[d(0.3)r(#2)]
*{\scriptstyle{#1}}
}
}

\def\gidbrn{ \gidbrv{n}{1} }
\def\gidbrnmtd{ \gidbrv{n-2d}{2} }
\def\cidbrn{ \bsymcat{\,\gidbrn} }
%\def\cIdbn{\cidbrn}


%********************************

\def\tstgrt{
\xygraph{
!{0;/r0.75pc/:}
!{\xcaph@(0)}
[d(1.5)l(1)]
!{\xcaph@(0)}
[u(1)l(0.4)]
*{\vdots}
[d(0.3)r(1)]
*{\scriptstyle{n}}
}
}

\def\tstgro{
\xygraph{
!{0;/r0.75pc/:}
!{\hcap-}
[u(0.5)]
*{\scriptstyle{i}}
[d(1)r(1)]
*{\scriptstyle{n}}
}
}

\def\testgr{
\underbrace{
\xygraph{
!{0;/r1.5pc/:}
%*+{n(n-2)}*\frm<8pt>{-,}
%[d(2)]
[] *+[F]{\;\;\scriptstyle{n}\;\;}
[l(0.5)d(0.4)]
!{\xcapv[0.5]@(0)}
[r(1)u(1)]
!{\xcapv[0.5]@(0)}
[u(2.3)]
!{\xcapv[0.5]@(0)}
[l(1)u(1)]
!{\xcapv[0.5]@(0)}
}
}_{n}
}

\def\testgr1{
\xygraph{
!{0;/r1.5pc/:}
!{\vtwist}
!{\vtwist}
}
}

\def\testgr2{
\xygraph{
!{0;/r0.75pc/:}
!{\hcrossneg}
!{\hcrossneg}
}
}

